A Semi-Decidable Procedure for Secrecy in Cryptographic Protocols

In this paper, we present a new semi-decidable procedure to analyze cryptographic protocols for secrecy based on a new class of functions that we call: the Witness-Functions. A Witness-Function is a reliable function that guarantees the secrecy in any protocol proved increasing once analyzed by it. Hence, the problem of correctness becomes a problem of protocol growth. A Witness-Function operates on derivative messages in a role-based specification and introduces new derivation techniques. We give here the technical aspects of the Witness-Functions and we show how to use them in a semi-decidable procedure. Then, we analyze a variation of the Needham-Schroeder protocol and we show that a Witness-Function can also help to teach about flaws. Finally, we analyze the NSL protocol and we prove that it is correct with respect to secrecy.

==> ConfProofsEK.tex <==
\begin{center}{\Large{\textbf{THE WITNESS-FUNCTIONS: PROOFS AND INTERMEDIATE RESULTS}}}\end{center}
$$\mbox{by: Jaouhar Fattahi, Mohamed Mejri and Hanane Houmani- April 2014}$$
$ $\\
\\
\section{Intermediate results and proofs for correctness of increasing protocols}
\subsection*{Valid trace}
Before defining a valid trace, let's give some intermediate definitions.\\

1- Step: it is defined by the following BNF grammar:
\[step :: \langle j.i, A \longrightarrow I (B) : m\rangle  | \langle j.i, I  (a) \longrightarrow B : m\rangle
\]

where $j$ is the identifier of the session and $i$ is the identifier of the step.\\

2- Trace: a trace $\rho$ is a sequence of steps. It is defined by the following BNF grammar:

\[\rho :: \varepsilon \mbox{ }| \mbox{ } step \mbox{ }|\mbox{ } \rho.step
\]

where $\varepsilon$ is the empty trace. We denote by $\bar{\rho}$ all the steps of $\rho$.\\

3- Session identifier: every step has an identifier. The set of identifiers ${\mathcal{S}}^{\rho}$ associated with a trace $\rho$ is built as follows:
\begin{center}
\begin{tabular}{r c l}
   ${\mathcal{S}}^{\varepsilon}$& $=$ & $\emptyset$ \\
   ${\mathcal{S}}^{\rho.\langle j.i,A\longrightarrow I(B):m\rangle }$& $=$ & ${\mathcal{S}^{\rho}}\cup \{j\}$ \\
   ${\mathcal{S}}^{\rho.\langle j.i,I (a)\longrightarrow B:m\rangle }$& $=$ & ${\mathcal{S}^{\rho}}\cup\{j\}$ \\
\end{tabular}
\end{center}

4- Session: a trace is an interleaving of many sessions where each of them has an identifier. We define a session (identified by ${Id}$) associated with a trace $\rho^n$ (coming from an interleaving of many sessions) as follows:

\begin{center}
\begin{tabular}{r c l c}
   ${\varepsilon}^{Id}$& $=$ & ${\varepsilon}$ \\
   $(\rho.\langle j.i,A\longrightarrow I(B):m\rangle )^{Id}$& $=$ & $\rho^{Id}$ &\mbox{      if } ${Id}\neq j$\\
   $(\rho.\langle j.i,I (a)\longrightarrow B:m\rangle )^{Id}$& $=$ & $\rho^{Id}$ &\mbox{      if } ${Id}\neq j$\\
   $(\rho.\langle {Id}.i,A\longrightarrow I(B):m\rangle )^{Id}$& $=$ & $\rho^{Id}.\langle {Id}.i,A\longrightarrow I(B):m\rangle $ \\
   $(\rho.\langle {Id}.i,I (a)\longrightarrow B:m\rangle )^{Id}$& $=$ & $\rho^{Id}.\langle {Id}.i,I (a)\longrightarrow B:m)\rangle $ \\

\end{tabular}
\end{center}

where $\varepsilon$ is the empty trace. It may be eliminated when preceded or followed by a non-empty trace.\\

5- $\mbox{Def}/\mbox{Use}$: the knowledge of the intruder change from a step to another. After an execution of  a trace, the intruder acquires new knowledge or defines herself news messages. We denote by $\mbox{Def}(\rho)$ the knowledge (messages) received by the intruder after execution of a trace $\rho$, and by $\mbox{Use}(\rho)$ the messages she builds after the execution of $\rho$. $\mbox{Use}(\rho)$ and $\mbox{Def}(\rho)$ are defined as follows:

\begin{center}
\begin{tabular}{r c l}
   $\mbox{Def}({\varepsilon})$& $=$ & $\emptyset$ \\
   $\mbox{Def}({\rho.\langle j.i,A\longrightarrow I(B):m\rangle })$& $=$ & $\mbox{Def}(\rho)\cup \{m\} $ \\
   $\mbox{Def}({\rho.\langle j.i,I (a)\longrightarrow B:m\rangle })$& $=$ & $\mbox{Def}(\rho)$ \\
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{r c l}
   $\mbox{Use}({\varepsilon})$& $=$ & $\emptyset$ \\
   $\mbox{Use}({\rho.\langle j.i,A\longrightarrow I(B):m\rangle })$& $=$ & $\mbox{Use}(\rho)$ \\
   $\mbox{Use}({\rho.\langle j.i,I (a)\longrightarrow B:m\rangle })$& $=$ & $\mbox{Use}(\rho)\cup \{m\} $  \\
\end{tabular}
\end{center}

For the sake of simplification, we denote by:
\begin{center} $\mbox{Use}(\rho)=\rho^+$ and $\mbox{Def}(\rho)=\rho^-$ \end{center}

6- ${\mathcal{C}}$-well-defined trace:
a trace is said ${\mathcal{C}}$-well-defined when the intruder is able to define all the messages contained in the trace before sending them. i.e for $\rho=\rho_1.e.\rho_2$ we have:
\[
{\rho_1}^+\models_{K(I)} e^-
\]
where $e$ is a step of communication and ${K(I)}$ are the knowledge of the intruder.\\

7- ${\mathcal{C}}$-well-formed trace: a trace is said ${\mathcal{C}}$-well-formed when it is generated by substitution in a generalized role of the protocol. ie, $\exists r \in R_G(p)$, a session $i\in {\mathcal{S}}^\rho$ and a substitution $\sigma\in \Gamma$ (the set of all substitutions) such that:
\[
{\rho}^{i}= r\sigma
\]

8- Valid trace: $\rho$ is a valid trace of a protocol $p$ when $\rho$ is ${\mathcal{C}}$-well-defined and $\rho$ is ${\mathcal{C}}$-well-formed.\\

A valid trace is a run of a protocol. It is an instance of the generalized roles produced by the intruder (or a regular agent) with respect to the rules of the protocol and the context of verification. 

\begin{defini}(Prefix of a trace)\label{PrefixeTrace}
$ $\\
Let $\rho_1$ and $\rho_2$ be two traces.
\begin{center}
$\rho_2$ is a prefix of $\rho_1$ if $\exists \rho_3$ such that: $\rho_1=\rho_2.\rho_3$
\end{center}
\end{defini}
\begin{defini}(Size of a trace)\label{TailleTrace}
$ $\\
The size of a trace $\rho$ denoted by $|\rho|$ is defined as follows:
\begin{center}
\begin{tabular}{rcl}
  % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
  $|{\varepsilon}|$ & $=$ & $0$ \\
  $|step|$ & $=$ & $1$ \\
  $|\rho.\rho'|$ & $=$ & $|\rho|+|\rho'|$  \\
\end{tabular}
\end{center}
\end{defini} 

%%% preuves du chapitre relatif au téhorème fondamental.

\begin{defini}(Well-formed interpretation function)\label{bienformeProofs}
$ $\\
Let $F$ be an interpretation function and ${\mathcal{C}}$ a context of verification. \\
$F$ is well-formed in ${\mathcal{C}}$ if:\index{Fonction well-formed}\\
$\forall M,M_1,M_2 \subseteq {\mathcal{M}}, \forall \alpha \in {\mathcal{A}}({\mathcal{M}}) \mbox{:}\\$
\[
\left\{
    \begin{array}{lll}
         F(\alpha,\{\alpha\})&= & \bot \\
         F(\alpha, {M}_1 \cup {M}_2)&= & F(\alpha, {M}_1)\sqcap F(\alpha,{M}_2) \\
         F(\alpha,{M})& =&\top, \mbox{ if } \alpha \notin {\mathcal{A}}({M})  \\
    \end{array}
\right.
\]
\end{defini}

For an atom $\alpha$ in a set of messages $M$, a well-formed interpretation function returns the bottom value "$\bot$", if $M=\{\alpha\}$. It returns for it in the union of two sets, the minimum "$\sqcap$" of the two values calculated in each set separately. It returns the top value "$\top$", if it does not appear in this set.

\begin{defini}(Full-invariant-by-intruder interpretation function)\label{spiProofs}
$ $\\
Let $F$ be an interpretation function and ${\mathcal{C}}$ a context of verification.  \index{Interpretation function}\\
$F$ is full-invariant-by-intruder in ${\mathcal{C}}$ if:\\
$
\forall {M} \subseteq {\mathcal{M}}, m\in {\mathcal{M}}. {M} \models_{\mathcal{C}} m \Rightarrow \forall \alpha \in {\mathcal{A}}(m). (F(\alpha,m) \sqsupseteq F(\alpha,{M}))  \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner)
$
\end{defini}

A reliable function $F$ should be full-invariant-by-intruder. That is to say, if $F$ attributes a security level  to a message $\alpha$ in $M$, then the intruder can never produce from $M$ another message $m$ that decrease this level  (i.e. $F(\alpha,m) \sqsupseteq F(\alpha,{M})$) except when $\alpha$ is intended to be known by the intruder (i.e. $\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner$).




\begin{defini}(Reliable interpretation function)\label{ReliableFunctionsProofs}
$ $\\
Let $F$ be an interpretation function and ${\mathcal{C}}$ a context of verification.
\[F  \mbox { is }{\mathcal{C}}\mbox{-reliable}  \mbox{ if } F \mbox{ is well-formed and } F \mbox{ is full-invariant-by-intruder in } {\mathcal{C}}.\]
\end{defini} 

A reliable interpretation function is simply a function that is well-formed and full-invariant-by-intruder in a given context of verification ${\mathcal{C}}$.


\begin{defini}($F$-increasing protocol)\label{ProAbsCroiProofs}
$ $\\
Let $F$ be an interpretation function, ${\mathcal{C}}$ a context of verification  and $p$ a protocol.\\
$p$ is $F$-increasing in ${\mathcal{C}}$ if:\\
$\forall R.r \in R_G(p),\forall \sigma \in \Gamma: {\mathcal{X}} \rightarrow {\mathcal{M}}_p  \mbox{ we have: }$
\[
\forall \alpha \in {\mathcal{A}}({\mathcal{M}}).F(\alpha, r^+\sigma)\sqsupseteq \ulcorner \alpha \urcorner \sqcap F(\alpha, R^-\sigma)
\]
\end{defini}

A $F$-increasing protocol produces  valid traces (interleaving of substituted generalized roles) where every involved principal (every substituted generalized role) never decreases the security levels of received components. When a protocol is  $F$-increasing and $F$ is a reliable function, it will be easy to prove its correctness with respect to the secrecy property. In fact, if every agent appropriately  protects her sent messages (if she initially knows the security level of a component, she has to encrypt it with at least one key having a similar or higher security level, and if she does not know its security level,  she estimates it using a reliable function), the intruder can never reveal it.



\begin{defini}(Secret disclosure)\label{divulgationProofs}
$ $\\
Let $p$ be a protocol and ${\mathcal{C}}$ a context of verification.\\
We say that $p$ discloses a secret $\alpha\in {\mathcal{A}}({\mathcal{M}})$  in ${{\mathcal{C}}}$ if:
%%\[
%%[\![p]\!] \models_{{\mathcal{C}}} \alpha\wedge(\ulcorner K(I) \urcorner \not \sqsupseteq \ulcorner \alpha \urcorner)
%%\]
%%\[ \mbox{i.e.} \]
\[\exists \rho\in [\![p]\!].(\rho \models_{{\mathcal{C}}} \alpha)\wedge(\ulcorner K(I) \urcorner \not \sqsupseteq \ulcorner \alpha \urcorner)\]
\end{defini}

A secret disclosure consists in exploiting a valid trace of the protocol (denoted by $ [\![p]\!]$) by the intruder using her knowledge $K(I) $ in a context of verification ${{\mathcal{C}}}$, to infer a secret $\alpha$ that she is not allowed to know (expressed by: $\ulcorner K(I) \urcorner \not \sqsupseteq \ulcorner \alpha \urcorner$).

\begin{defini}(${\mathcal{C}}$-correct protocol with respect to the secrecy property)\label{correctionProofs}
$ $\\
Let $p$ be a protocol and ${\mathcal{C}}$ a context of verification. \\
$p$ is ${\mathcal{C}}$-correct with respect to the secrecy property  if:
\[
\forall \alpha\in {\mathcal{A}}({\mathcal{M}}), \forall \rho \in [\![p]\!]. \rho \models_{{\mathcal{C}}} \alpha \Rightarrow \ulcorner K(I) \urcorner  \sqsupseteq \ulcorner \alpha \urcorner
\]
We denote:
\[\forall \alpha\in {\mathcal{A}}({\mathcal{M}}). [\![p]\!] \models_{\mathcal{C}}  \alpha \Rightarrow \ulcorner K(I) \urcorner  \sqsupseteq \ulcorner \alpha \urcorner
\]

\end{defini}

A correct protocol is such that any valid trace $\rho$ that it produces never leaks a secret that the intruder is not allowed to know. %%That is to say, if the protocol produces a valid trace that the intruder can exploit using the context of verification to deduce an atomic message $\alpha$ then her knowledge $K(I)$ are initially greater than this atom, which means that she is initially allowed to know.




\begin{defini}($\sqsupseteq_F$)\label{RelatSupF}
$ $\\
$ $\\
Let ${\mathcal{C}}=\langle{\mathcal{M}},\xi,\models,{\mathcal{K}},{\mathcal{L}}^\sqsupseteq,\ulcorner .\urcorner\rangle$ be a verification context.\\
Let $F$ be an interpretation function. \index{Interpretation function}\\
Let $M_1$, $M_2$ $\subseteq$ ${\mathcal{M}}$.\\
\[
M_1 \sqsupseteq_F M_2 \Longleftrightarrow \forall \alpha \in {\mathcal{A}}(M_1).F(\alpha,M_1) \sqsupseteq F(\alpha,{M_2})
\]

\end{defini}

\begin{defini}(Auxiliary Interpretation function)\label{bienformederivee}\index{Interpretation function}
$ $\\
$ $\\
Let ${\mathcal{C}}=\langle{\mathcal{M}},\xi,\models,{\mathcal{K}},{\mathcal{L}}^\sqsupseteq,\ulcorner .\urcorner\rangle$ be a verification context.\\
Let $F$ be an interpretation function.\\
We define the auxiliary function of $F$, denoted by $\hat{F}$, as follows:
\[
\begin{array}{cccc}
  \hat{F}: & {\mathcal{A}}\times {\mathcal{M}} & \longmapsto & {\mathcal{L}}^\sqsupseteq \\
   & (\alpha,m) & \longmapsto & \ulcorner\alpha\urcorner \sqcap F(\alpha,m)
\end{array}
\]

\end{defini}

\begin{defini}($\sqsupseteq_{\hat{F}}$)\label{RelatSupHatF}
$ $\\
$ $\\
Let ${\mathcal{C}}=\langle{\mathcal{M}},\xi,\models,{\mathcal{K}},{\mathcal{L}}^\sqsupseteq,\ulcorner .\urcorner\rangle$ be a verification context.\\
Let $F$ be an interpretation function. \index{Interpretation function}\\
Let $M_1$, $M_2$ $\subseteq$ ${\mathcal{M}}$\\
\[
M_1 \sqsupseteq_{\hat{F}} M_2 \Longleftrightarrow \forall \alpha \in {\mathcal{A}}(M_1).{\hat{F}}(\alpha,M_1) \sqsupseteq {\hat{F}}(\alpha,{M_2})
\]
\end{defini}

\begin{pre}
$ $\\
$ $\\
Let ${\mathcal{C}}=\langle{\mathcal{M}},\xi,\models,{\mathcal{K}},{\mathcal{L}}^\sqsupseteq,\ulcorner .\urcorner\rangle$ be a verification context.\\
Let $F$ be an interpretation function.\\
Let $\hat{F}$ be the auxiliary function of $F$.\\
\\
If $F$ is well-formed in ${\mathcal{C}}$ then:
\\
\\
$\forall M,M_1,M_2 \subseteq {\mathcal{M}}, \forall \alpha \in {\mathcal{A}}({\mathcal{M}}).\\$
\[
\left\{
    \begin{array}{lll}
         \hat{F}(\alpha,\{\alpha\})&= & \bot \\
         &\mbox{and} &\\
         \hat{F}(\alpha, {M}_1 \cup {M}_2)&= & \hat{F}(\alpha, {M}_1)\sqcap \hat{F}(\alpha,{M}_2) \\
         &\mbox{and} &\\
         \hat{F}(\alpha,{M})& =&\ulcorner\alpha\urcorner, \mbox{ if } \alpha \notin {\mathcal{A}}({M})  \\
    \end{array}
\right.
\]

\end{pre}
$ $\\
See the proof \ref{PR1}.


\begin{preuve}\label{PR1}
$ $\\
$ $\\
$F$ is well-formed in ${\mathcal{C}}$ then we have from the definition \label{bienformeProofs}:
\\
\\
$\forall M,M_1,M_2 \subseteq {\mathcal{M}}, \forall \alpha \in {\mathcal{A}}({\mathcal{M}}).\\$
\begin{equation}
\left\{
    \begin{array}{lll}
         F(\alpha,\{\alpha\})&= & \bot \\
         &\mbox{and} &\\
         F(\alpha, {M}_1 \cup {M}_2)&= & F(\alpha, {M}_1)\sqcap F(\alpha,{M}_2) \\
         &\mbox{and} &\\
         F(\alpha,{M})& =&\top, \mbox{ if } \alpha \notin {\mathcal{A}}({M})  \\
    \end{array}
\right.\label{eq1bienformee}
\end{equation}
From \ref{eq1bienformee}, we have the three following results:
\begin{itemize}
  \item [$\bullet$]\begin{equation}F(\alpha,\{\alpha\})=\bot \label{eq2bienformee}\end{equation}
  From \ref{eq2bienformee} and since ${\mathcal{L}}^\sqsupseteq$ is a lattice, we have:
  \begin{equation}\ulcorner\alpha\urcorner \sqcap F(\alpha,\{\alpha\})=\bot \label{biseq2bienformee}\end{equation}
  From \ref{biseq2bienformee} and the definition \ref{bienformederivee} of $\hat{F}$ we have:
  \begin{equation}\hat{F}(\alpha,\{\alpha\})=\bot \label{biseq3bienformee}\end{equation}
  \item [$\bullet$]\begin{equation}F(\alpha, {M}_1 \cup {M}_2)=F(\alpha, {M}_1)\sqcap F(\alpha,{M}_2)\label{biseq4bienformee}\end{equation}
  From \ref{biseq4bienformee} and since ${\mathcal{L}}^\sqsupseteq$ is a lattice we have:
    \begin{equation}\ulcorner\alpha\urcorner \sqcap F(\alpha, {M}_1 \cup {M}_2)=\ulcorner\alpha\urcorner\sqcap (F(\alpha, {M}_1)\sqcap F(\alpha,{M}_2))\label{biseq5bienformeeModi}\end{equation}
  Or else:
  \begin{equation}\ulcorner\alpha\urcorner \sqcap F(\alpha, {M}_1 \cup {M}_2)=\ulcorner\alpha\urcorner\sqcap F(\alpha, {M}_1)\sqcap \ulcorner\alpha\urcorner\sqcap F(\alpha,{M}_2)\label{biseq5bienformee}\end{equation}

  From \ref{biseq5bienformee} and from the definition \ref{bienformederivee} of $\hat{F}$ we have:
  \begin{equation}\hat{F}(\alpha, {M}_1 \cup {M}_2)=\hat{F}(\alpha, {M}_1)\sqcap \hat{F}(\alpha,{M}_2)\label{biseq6bienformee}\end{equation}

  \item [$\bullet$]\begin{equation}F(\alpha,{M})=\top \mbox{, if } \alpha \notin {M}\label{eq4bienformee}\end{equation}
  From \ref{eq4bienformee} and since ${\mathcal{L}}^\sqsupseteq$ is a lattice and $\ulcorner\alpha\urcorner \sqsubseteq \top$ we have:
      \begin{equation}\ulcorner\alpha\urcorner\sqcap F(\alpha,{M})=\ulcorner\alpha\urcorner \mbox{, if } \alpha \notin {\mathcal{A}}(M)\label{biseq7bienformee}\end{equation}
  From \ref{biseq7bienformee} and from the definition \ref{bienformederivee} of $\hat{F}$ we have:
  \begin{equation}\hat{F}(\alpha,{M})=\ulcorner\alpha\urcorner \mbox{, if } \alpha \notin {\mathcal{A}}(M)\label{biseq8bienformee}\end{equation}
\end{itemize}
From \ref{biseq3bienformee}, \ref{biseq6bienformee} and \ref{biseq8bienformee} we have:\\
\\
$\forall M,M_1,M_2 \subseteq {\mathcal{M}}, \forall \alpha \in {\mathcal{A}}({\mathcal{M}}).\\$
\[
\left\{
    \begin{array}{lll}
         \hat{F}(\alpha,\{\alpha\}&= & \bot \\
         &\mbox{and} &\\
         \hat{F}(\alpha, {M}_1 \cup {M}_2)&= & \hat{F}(\alpha, {M}_1)\sqcap \hat{F}(\alpha,{M}_2) \\
         &\mbox{and} &\\
         \hat{F}(\alpha,{M})& =&\ulcorner\alpha\urcorner, \mbox{ if } \alpha \notin {\mathcal{A}}({M})  \\
    \end{array}
\right.
\]
\end{preuve}


\begin{pre}
$ $\\
$ $\\
Let ${\mathcal{C}}=\langle{\mathcal{M}},\xi,\models,{\mathcal{K}},{\mathcal{L}}^\sqsupseteq,\ulcorner .\urcorner\rangle$ be a verification context.\\
Let $F$ be an interpretation function.\\
Let $\hat{F}$ the auxiliary function of $F$.\\
If $F$ is full-invariant-by-intruder in ${\mathcal{C}}$ then $\hat{F}$ is full-invariant-by-intruder in ${\mathcal{C}}$.
\end{pre}
$ $\\
See the proof \ref{PR2}.

\begin{preuve}\label{PR2}
$ $\\
$ $\\
Let ${M} \subseteq {\mathcal{M}}$ and $m \in {\mathcal{M}}$ such that:
\begin{equation}
 {M} \models_{{\mathcal{C}}} m
\label{eq1spihatModif}
\end{equation}
From the definition \ref{spiProofs} and \ref{eq1spihatModif} we have for all $\alpha\in {\mathcal{A}}(m)$:\\
\begin{equation}
(F(\alpha,m) \sqsupseteq F(\alpha,{M}))  \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner)\label{eq1spihat}
\end{equation}
From \ref{eq1spihat} we have:\\
\begin{itemize}
  \item [$\bullet$]either: \begin{equation}F(\alpha,m) \sqsupseteq F(\alpha,{M})\label{eq3spihat}
\end{equation}
From \ref{eq3spihat} and since ${\mathcal{L}}^\sqsupseteq$ is a lattice, we have:\\
 \begin{equation}\ulcorner \alpha \urcorner \sqcap F(\alpha,m) \sqsupseteq \ulcorner \alpha \urcorner \sqcap F(\alpha,{M})\label{eq5spihat}
\end{equation}
From \ref{eq5spihat} and from the definition \ref{bienformederivee} de $\hat{F}$ we have:
 \begin{equation}\hat{F}(\alpha,m) \sqsupseteq \hat{F}(\alpha,{M})\label{eq6spihat}
\end{equation}
  \item [$\bullet$] or: \begin{equation}\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner\label{eq7spihat}
\end{equation}
\end{itemize}
From \ref{eq6spihat} and \ref{eq7spihat} we have for all ${M} \subseteq {\mathcal{M}}$ and $m \in {\mathcal{M}}$:\\
\[
 {M} \models_{{\mathcal{C}}} m \Rightarrow \forall \alpha \in {\mathcal{A}}(m). (\hat{F}(\alpha,m) \sqsupseteq \hat{F}(\alpha,{M}))  \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner)
\]
Then $\hat{F}$ is full-invariant-by-intruder in ${\mathcal{C}}$.
\end{preuve}


\begin{lem}\label{lem411Proofs}
$ $\\
$ $\\
Let ${\mathcal{C}}=\langle{\mathcal{M}},\xi,\models,{\mathcal{K}},{\mathcal{L}}^\sqsupseteq,\ulcorner .\urcorner\rangle$ be a verification context.\\
Let $F$ be a ${\mathcal{C}}$-reliable interpretation function.\\
Let $p$ be a protocol.\\
\\
We have:\\

If ($p$ is $F$-increasing in ${\mathcal{C}}$)$ \mbox{ then } (\forall \rho.e \in [\![p]\!]\mbox{ we have: }e^+\sqsupseteq_{\hat{F}} \rho^-)$

\end{lem}
$ $\\
See the proof \ref{PR3}.

\begin{preuve}\label{PR3}
$ $\\
$ $\\
Since $p$ is an $F$-increasing protocol in ${\mathcal{C}}$, then from the definition \ref{ProAbsCroiProofs} we have:\\
\\
$\forall R.r \in R_G(p), \forall \sigma\in \Gamma: X \rightarrow {\mathcal{M}}_p(closed)$ we have:\\
\begin{equation}\forall \alpha \in {{\mathcal{A}}(r^+\sigma)}.F(\alpha, r^+\sigma)\sqsupseteq \ulcorner \alpha \urcorner \sqcap F(\alpha, R^-\sigma)\label{eq1trace}\end{equation} \\
Since $\rho.e$ is a valid trace, then exists a substitution $\sigma\in \Gamma$, a generalized role $R.r$ $\in R_G(p)$ and a session $i=S(e)$ such that:
\begin{equation}(R\sigma=\rho^i)\wedge(r\sigma=e) \label{eq2trace}\end{equation}
From \ref{eq1trace} and \ref{eq2trace}, we have:
\begin{equation}\forall \alpha \in {\mathcal{A}}(e^+).F(\alpha,e^+)\sqsupseteq \ulcorner \alpha \urcorner \sqcap F(\alpha,\rho^{i-})\label{eq3trace}\end{equation}
Since ${\mathcal{L}}^\sqsupseteq$ is a lattice, we have:
\begin{equation}\forall \alpha \in {\mathcal{A}}(e^+).\ulcorner \alpha \urcorner \sqcap F(\alpha,e^+)\sqsupseteq \ulcorner \alpha \urcorner \sqcap \ulcorner \alpha \urcorner \sqcap F(\alpha,\rho^{i-})\label{eq4trace}\end{equation}
From \ref{eq4trace} and since ${\mathcal{L}}^\sqsupseteq$ is a lattice we have:
\begin{equation}\forall \alpha \in {\mathcal{A}}(e^+).\ulcorner \alpha \urcorner \sqcap F(\alpha,e^+)\sqsupseteq \ulcorner \alpha \urcorner \sqcap F(\alpha,\rho^{i-})\label{eq5trace}\end{equation}
From the definition of $\hat{F}$ and from \ref{eq5trace}, we have:
\begin{equation}\forall \alpha \in {\mathcal{A}}(e^+). \hat{F}(\alpha,e^+)\sqsupseteq \hat{F}(\alpha,\rho^{i-}) \label{eq6trace}\end{equation}
From \ref{eq6trace} and the definition of $\sqsupseteq_{\hat{F}}$, we have:
\begin{equation}e^+\sqsupseteq_{\hat{F}}\rho^{i-}\label{eq7trace}\end{equation}
Since $\mbox{Use}(\rho^{i})\subseteq \mbox{Use}(\rho) $, from the definition of $\sqsupseteq_{\hat{F}}$ and since ${\mathcal{L}}^\sqsupseteq$ is a lattice, then we have:
\begin{equation}\rho^{i-} \sqsupseteq_{\hat{F}} \rho^-\label{eq8trace}\end{equation}
From \ref{eq7trace} and \ref{eq8trace}, we deduce that:
 \[e^+ \sqsupseteq_{\hat{F}} \rho^-\]


\end{preuve}

\begin{lem}\label{lemprincProofs}
$ $\\
Let $F$ be a ${\mathcal{C}}$-reliable interpretation function and $p$ a $F$-increasing protocol.\\
We have:
\[
\forall m \in {\mathcal{M}}. [\![p]\!] \models_{\mathcal{C}} m \Rightarrow \forall \alpha \in {\mathcal{A}}(m). (F(\alpha,m)\sqsupseteq \ulcorner \alpha \urcorner)\vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner).
\]

\end{lem}

The lemma \ref{lemprincProofs} asserts that for any atom $\alpha$ in a message generated by an increasing protocol, its security level calculated by a reliable interpretation function is maintained greater than its initial value in the context, if the intruder is not initially allowed to know it. Thus, initially the atom has a certain security level. This value cannot be decreased by the intruder using her initial knowledge and received messages since reliable functions are full-invariant-by-intruder. In each new step of any valid trace, involved messages are better protected since the protocol is increasing.  The proof is run by induction on the size of the trace and uses the reliability properties of the interpretation function in every step.\\
$ $\\
\\
See the proof \ref{PR4}

\begin{preuve}\label{PR4}
$ $\\
$ $\\
Let $\rho\in [\![p]\!]$ and $m \in {\mathcal{M}}$ such that: \begin{equation}\rho^+ \models_{\mathcal{C}} m \label{eq1preuvesti}\end{equation}
Let's prove the lemma by induction on the size of the trace.\\
\begin{itemize}
\item [$\bullet$] $|\rho|$=1.\\
\\
In this case, we have two sub-cases:\\
\begin{itemize}
\item[$\bullet$] either $\rho^+=\emptyset$, and so we have:\\
\\
From \ref{eq1preuvesti}, we have: \begin{equation}\emptyset \models_{\mathcal{C}} m\label{eq2preuvesti}\end{equation}
Since $F$ is full-invariant-by-intruder in ${\mathcal{C}}$, we have:
\begin{equation}\forall \alpha \in {\mathcal{A}}(m).(F(\alpha,m) \sqsupseteq F(\alpha,\emptyset))  \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{eq3preuvesti}\end{equation}
Since $\alpha \notin \emptyset$ and $F$ is well-formed in ${\mathcal{C}}$, we have: \begin{equation}F(\alpha,\emptyset)=\top \sqsupseteq \ulcorner \alpha \urcorner\label{eq4preuvesti}\end{equation}
From \ref{eq3preuvesti}  and \ref{eq4preuvesti}, we have:
\begin{equation}\forall \alpha \in {\mathcal{A}}(m).(F(\alpha,m) \sqsupseteq \ulcorner \alpha \urcorner)  \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{eq5preuvesti}\end{equation}
\end{itemize}
\begin{itemize}
\item[$\bullet$] or $\rho^+\neq\emptyset$, and so we have:
\newline
\newline
Since $|\rho|$=1 then exists an empty trace $\varepsilon$ such that $\rho=\varepsilon\rho^+$
\newline
\\
Since $F$ is full-invariant-by-intruder in ${\mathcal{C}}$, we have:\\
\begin{equation}\forall \alpha \in {\mathcal{A}}(m).(F(\alpha,m) \sqsupseteq F(\alpha,\rho^+))  \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner)\label{eq6preuvesti}\end{equation}
Since $p$ is $F$-increasing in ${\mathcal{C}}$, then from the lemma~\ref{lem411Proofs}, we have:
\begin{equation}\rho^+\sqsupseteq_{\hat{F}} \varepsilon^-\label{eq7preuvesti}\end{equation}
Or else: \begin{equation}\forall \alpha \in {\mathcal{A}}(\rho^+).\hat{F}(\alpha,\rho^+) \sqsupseteq
\hat{F}(\alpha,\varepsilon^-)\label{eq8preuvestibis}\end{equation}
\newline
From \ref{eq8preuvestibis} and from the definition of $\hat{F}$ we have: \begin{equation}\forall \alpha \in {\mathcal{A}}(\rho^+).F(\alpha,\rho^+) \sqcap \ulcorner \alpha \urcorner \sqsupseteq \hat{F}(\alpha,\varepsilon^-)\label{eq8preuvesti}\end{equation}
Since $\varepsilon$ is an empty trace and $\hat{F}$ is well-formed in ${\mathcal{C}}$, then: \begin{equation}\hat{F}(\alpha,\varepsilon^-)=\ulcorner \alpha \urcorner\label{eq8preuvestiih}\end{equation}
From \ref{eq8preuvesti} and \ref{eq8preuvestiih} we have:
\begin{equation}\forall \alpha \in {\mathcal{A}}(\rho^+).F(\alpha,\rho^+) \sqcap \ulcorner \alpha \urcorner \sqsupseteq \ulcorner \alpha \urcorner\label{eq8preuvestiModMod1}\end{equation}
Since ${\mathcal{L}}^\sqsupseteq$ is a lattice, we have:
\begin{equation}\forall \alpha \in {\mathcal{A}}(\rho^+).F(\alpha,\rho^+) \sqsupseteq F(\alpha,\rho^+) \sqcap \ulcorner \alpha \urcorner\label{eq8preuvestiModMod2}\end{equation}
From \ref{eq8preuvestiModMod1} and \ref{eq8preuvestiModMod2}, we have: \begin{equation}\forall \alpha \in {\mathcal{A}}(\rho^+).F(\alpha,\rho^+) \sqsupseteq \ulcorner \alpha \urcorner\label{eq9preuvesti}\end{equation}
We deduce from \ref{eq6preuvesti} and \ref{eq9preuvesti}:
\begin{equation}\forall \alpha \in {\mathcal{A}}(m).(F(\alpha,m) \sqsupseteq \ulcorner \alpha \urcorner)  \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner)\label{eq10preuvesti}\end{equation}
\end{itemize}
\end{itemize}
\begin{itemize}
\item [$\bullet$]We assume for $|\rho|\le n$, we have:
\begin{equation}\forall \alpha \in {\mathcal{A}}(m).(F(\alpha,m) \sqsupseteq \ulcorner \alpha \urcorner)  \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner)\label{eq11preuvesti}\end{equation}
Let's prove that for $|\rho|=n+1$, we have:
\begin{equation}\forall \alpha \in {\mathcal{A}}(m).(F(\alpha,m) \sqsupseteq \ulcorner \alpha \urcorner)  \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner)\label{eq12preuvesti}\end{equation}
Let $m \in {\mathcal{M}}$ such that $\rho^+ \models_C m $ with $|\rho|=n+1$.\\
\\
Let $\rho=\rho_n.e$\\
  \\
Since  $|\rho|=n+1$, we have: \begin{equation}|\rho_n|\leqslant n \mbox{ and } |e|\leqslant n \label{eq13preuvesti}\end{equation}
  From \ref{eq11preuvesti} and \ref{eq13preuvesti} and since $\rho_n^+\models_{\mathcal{C}}\rho_n^+$ and $e^+\models_{\mathcal{C}}e^+$ we have:
  \begin{equation} \forall \alpha \in {\mathcal{A}}(\rho_n^+).(F(\alpha,\rho_n^+) \sqsupseteq \ulcorner \alpha \urcorner)  \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{eq14preuvesti}\end{equation}
  $$\mbox{and}$$ \begin{equation} \forall \alpha \in {\mathcal{A}}(e^+).(F(\alpha,e^+) \sqsupseteq \ulcorner \alpha \urcorner)  \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{eq15preuvesti}\end{equation}
  From \ref{eq14preuvesti}, \ref{eq15preuvesti} and since $F$ is well-formed and ${\mathcal{L}}^\sqsupseteq$ is a lattice we have:
  \begin{equation} \forall \alpha \in {\mathcal{A}}(\rho_n^+\cup e^+).(F(\alpha,\rho_n^+)\sqcap F(\alpha,e^+) \sqsupseteq \ulcorner \alpha \urcorner)  \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{eq16preuvesti}\end{equation}

Since $F$ is full-invariant-by-intruder in ${\mathcal{C}}$ and $\rho^+\models_{\mathcal{C}} m$, then: \begin{equation}\forall \alpha \in {\mathcal{A}}(m). (F(\alpha,m)\sqsupseteq F(\alpha,\rho^+))\vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{eq17preuvesti}\end{equation}
  Since: \begin{equation}\rho^+=\rho_n^+ \cup e^+\label{eq18preuvesti}\end{equation}
 Then from \ref{eq18preuvesti} and since ${\mathcal{L}}^\sqsupseteq$ is a lattice we have:
  \begin{equation}\forall \alpha \in {\mathcal{A}}(\rho^+). F(\alpha,\rho^+) = F(\alpha,\rho_n^+) \sqcap F(\alpha,e^+) \label{eq19preuvesti}\end{equation}
 From \ref{eq16preuvesti} and \ref{eq19preuvesti}  we have:
  \begin{equation}\forall \alpha \in {\mathcal{A}}(\rho^+). (F(\alpha,\rho^+)\sqsupseteq \ulcorner \alpha \urcorner)\vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{eq20preuvesti}\end{equation}
  From \ref{eq17preuvesti} and \ref{eq20preuvesti} we have:\\
  \begin{equation}\forall \alpha \in {\mathcal{A}}(m). (F(\alpha,m)\sqsupseteq \ulcorner \alpha \urcorner)\vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{eq21preuvesti}\end{equation}

\end{itemize}
  From \ref{eq10preuvesti}, the induction assumption in \ref{eq11preuvesti} and from \ref{eq21preuvesti}, we have: for all $m \in {\mathcal{M}}$ and all $\rho \in [\![p]\!]$:
  \[
  \rho \models_{\mathcal{C}} m \Rightarrow (\forall \alpha \in {\mathcal{A}}(m). (F(\alpha,m)\sqsupseteq \ulcorner \alpha \urcorner)\vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner))
  \]
  Or else:
  \[
\forall m \in {\mathcal{M}}. [\![p]\!] \models_{\mathcal{C}} m \Rightarrow \forall \alpha \in {\mathcal{A}}(m).(F(\alpha,m)\sqsupseteq \ulcorner \alpha \urcorner)\vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner)
\]



\end{preuve}

\begin{thm}(Correctness of increasing protocols)\label{mainThmouchArticleProofs}
$ $\\
Let $F$ be a ${\mathcal{C}}$-reliable interpretation function and $p$ a $F$-increasing protocol.
\begin{center}
$p$ is ${\mathcal{C}}$-correct with respect to the secrecy property.
\end{center}\index{Confidentialité}


\end{thm}
$ $\\
See the proof \ref{PR5}

\begin{preuve}\label{PR5} 
$ $\\
Let's suppose that $p$ discloses an atomic secret $\alpha$. \\
\\
From the definition \ref{divulgationProofs} we have:
\begin{equation}\exists \rho\in [\![p]\!].(\rho \models_{\mathcal{C}} \alpha)\wedge(\ulcorner K(I) \urcorner \not \sqsupseteq \ulcorner \alpha \urcorner) \label{preuvthe1}\end{equation}
Since $F$ is a  ${\mathcal{C}}$-reliable interpretation function and $p$ an $F$-increasing protocol, we have from the lemma \ref{lemprincProofs}:
\begin{equation}(F(\alpha,\alpha)\sqsupseteq \ulcorner \alpha \urcorner)\vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner)\label{preuvthe2}\end{equation}
From \ref{preuvthe1} and \ref{preuvthe2}, we have:
\begin{equation}F(\alpha,\alpha)\sqsupseteq \ulcorner \alpha \urcorner \label{preuvthe3}\end{equation}
Since $F$ is well-formed in ${\mathcal{C}}$, then:
\begin{equation}F(\alpha,\alpha)= \bot \label{preuvthe4}\end{equation}
From \ref{preuvthe3} and \ref{preuvthe4} we have:
\begin{equation}\bot= \ulcorner \alpha \urcorner \label{preuvthe5cor}\end{equation}
\ref{preuvthe5cor} is impossible because it is contradictory with:  $\ulcorner K(I) \urcorner \not \sqsupseteq \ulcorner \alpha \urcorner$ in \ref{preuvthe1}.\\
\\
Then $p$ is ${\mathcal{C}}$-correct with respect to the secrecy property 
\end{preuve} 
%%\end{comment}
%%\pagebreak

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Intermediate results and proofs for well-protected messages}
%%% preuves du chapitre de construction des selection et fonctions fiables.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{defini}(${\mathcal{C}}$-encryption)\label{HanenBienProtege}
$ $\\
\begin{comment}
Let $M,M'\subseteq {\mathcal{M}}$, $f \in \Sigma$  and $m \in {\mathcal{M}}$.\\
\\
$f_k$ is a ${\mathcal{C}}$-encryption if the two following conditions are met:\\
$ $\\
$1-\mbox{ If }M\cup \{f_k(m)\}\models_{\mathcal{C}} m  \mbox{ and } M \not \models_{\mathcal{C}} m$ then $M\models_{\mathcal{C}} k^{-1}$
[Having the decryption key of an encrypted message is a pre-condition to obtain the message]
$ $\\
\\
$2-\mbox{ If }M\cup M'\models_{\mathcal{C}} f_k(m) \mbox{ and } M \not \models_{\mathcal{C}} f_k(m) \mbox{ and } M' \not \models_{\mathcal{C}} f_k(m)$ then $M \cup M' \models_{\mathcal{C}} m \mbox{ and } M \cup M' \models_{\mathcal{C}} k$
[Having the message and the encryption key are two preconditions to encrypt a message ]\\
\end{comment}
%%[Avoir le message and la clé sont deux conditions pour avoir le message encrypté]\\

We denote by ${\mathcal{E}}_{\mathcal{C}}$ the set of ${\mathcal{C}}$-encryption functions and by $\overline{{\mathcal{E}}}_{\mathcal{C}}$ the complementary set $\Sigma\backslash{\mathcal{E}}_{\mathcal{C}}$.

%%On note par ${\mathcal{E}}_{\mathcal{C}}$ l'ensemble from fonctions d'encryption dans ${\mathcal{C}}$ and par $\overline{{\mathcal{E}}}_{\mathcal{C}}$ l'ensemble complémentaire $\Sigma\backslash{\mathcal{E}}_{\mathcal{C}}$.
%%si $f_k$ is une ${\mathcal{C}}$-encryption and $(f:\overline{e})$ sinon.
%%On note $(f_k:e)$ si $f_k$ is une ${\mathcal{C}}$-encryption and $(f:\overline{e})$ sinon.

\end{defini}



\begin{defini}(Keys)\label{keysProofs}
$ $\\
$ $\\
Let $M\subseteq {\mathcal{M}}$, $f \in \Sigma$ and $m \in M$.\\
\\
%%On définit l'applicatiwe hwithcesseur as follows:\\
We define the application Keys as follows:
\[
\begin{tabular}{llll}
  $Keys:$ & ${\mathcal{A}}\times {\mathcal{M}}$ & $\longrightarrow$ & ${\mathcal{P}}({\mathcal{P}}({\mathcal{A}}))$\\
\end{tabular}
\]
$\forall t_1, t_2... t_n$ subterms of $m$:
\[
\begin{tabular}{lll}
  $Keys(\alpha,\alpha)$ & $=\{\emptyset\}$ &\\
  $Keys(\alpha,\beta)$ & $=\emptyset$,\mbox{ if } $\alpha \neq \beta$ $\mbox{ and } \beta \in {\mathcal{A}}$\\
  $Keys(\alpha,f_k(t_1,...,t_n))$ & $=\{k\} \otimes \overset{n}{\underset {i=1}{\cup}}Keys(\alpha,t_i),$ \mbox{if } $f_k \in {\mathcal{E}}_{\mathcal{C}}$ %%\mbox{ and } $f_k(t_1,...,t_n)=f_k(t_1,...,t_n)_\Downarrow$
  &\\
  $Keys(\alpha,f(t_1,...,t_n))$  &$=\overset{n}{\underset {i=1}{\cup}}Keys(\alpha,t_i),$$\mbox{ if } f\in\overline{{\mathcal{E}}}_{\mathcal{C}}$ %% $\mbox{ and } f_k(t_1,...,t_n)=f_k(t_1,...,t_n)_\Downarrow$
  &
 %% $Keys(\alpha,f(t_1,...,t_n))$  &$=Keys(\alpha,f(t_1,...,t_n)_\Downarrow)$,\mbox{ if not. }\\
\end{tabular}
\]
We extend the application $Keys$ to sets as follows:\\
\[
\forall M \subseteq {\mathcal{M}}. Keys(\alpha,M)=\underset {m \in M}{\cup}Keys(\alpha,m) \mbox{ and } Keys(\alpha,\emptyset)=\emptyset.
\]
\end{defini}
The application $keys$ defined in \ref{keysProofs} returns the keys of encryption of any atom $\alpha$ in a message $m$.

\begin{defini}(Equational theory, rewriting system and normal form)\label{normalform}
$ $\\
\\
We transform the equational theory $\xi$ given in the context to a convergent rewriting system $\rightarrow_{\xi}$ such that:
\begin{equation}
\forall m \in {\mathcal{M}},\forall \alpha \in {\mathcal{A}}(m), \forall l \rightarrow r \in \rightarrow_{\xi}, ~~~~~~~~~~Keys(\alpha,r) \subseteq Keys(\alpha,l) 
\end{equation}
We denote by $m_\Downarrow$ the normal form of $m$ in $\xi$.\\
\end{defini}
The normal form defined in \ref{normalform} is oriented such that it takes the form of a message having the minimum keys of encryption (the least protected form) and ignores the other forms having unnecessary keys of encryption. This kind of orientation poses no problem with the most of equational theories of the intruder in the literature.

\begin{exemple}
$$e(k,d(k^{-1},\alpha))\rightarrow \alpha$$
\end{exemple}

\begin{defini}(Accessor)
$ $\\
$ $\\
Let $M\subseteq {\mathcal{M}}$, $f \in \Sigma$ and $m \in M$.\\
%%On définit l'applicatiwe hwithcesseur as follows:\\
We define the application Accessor as follows:
\[
\begin{tabular}{llll}
  $Access:$ & ${\mathcal{A}}\times {\mathcal{M}}$ & $\longrightarrow$ & ${\mathcal{P}}({\mathcal{P}}({\mathcal{A}}))$\\
\end{tabular}
\]
$\forall t_1, t_2... t_n$ subterms of $m$:
\[
\begin{tabular}{lll}
  $Access(\alpha,\alpha)$ & $=\{\emptyset\}$ &\\
  $Access(\alpha,\beta)$ & $=\emptyset$,\mbox{ if } $\alpha \neq \beta$ $\mbox{ and } \beta \in {\mathcal{A}}$\\
  $Access(\alpha,f_k(t_1,...,t_n))$ & $=\{k^{-1}\} \otimes \overset{n}{\underset {i=1}{\cup}}Access(\alpha,t_i),$ \mbox{if } $f_k \in {\mathcal{E}}_{\mathcal{C}}$ \mbox{ and } $f_k(t_1,...,t_n)=f_k(t_1,...,t_n)_\Downarrow$
  &\\
  $Access(\alpha,f(t_1,...,t_n))$  &$=\overset{n}{\underset {i=1}{\cup}}Access(\alpha,t_i),$$\mbox{ if } f\in\overline{{\mathcal{E}}}_{\mathcal{C}}  \mbox{ and }$$f_k(t_1,...,t_n)=f_k(t_1,...,t_n)_\Downarrow$
  &\\
  $Access(\alpha,f(t_1,...,t_n))$  &$=Access(\alpha,f(t_1,...,t_n)_\Downarrow)$,\mbox{ if not. }\\
\end{tabular}
\]
We extend the application $Access$ to sets as follows:\\
\[
\forall M \subseteq {\mathcal{M}}. Access(\alpha,M)=\underset {m \in M}{\cup}Access(\alpha,m) \mbox{ and } Access(\alpha,\emptyset)=\emptyset.
\]
\end{defini}

Every element of $Access(\alpha,m)$ contains a set of required keys to decrypt $\alpha$ in $m$ after elimination of  unnecessary keys by the normal form. %%Please notice that $m$ is put in its normal form denoted by $m_\Downarrow$ before any step in $Access(\alpha,m)$.
\normalsize
\begin{exemple}
$ $\\
\\
Let $m$ be a message such that: $m=\{ \{ A.D.\alpha \}_{k_{ab}}.\alpha.\{ A.E.\{C.\alpha\}_{k_{ef}} \}_{k_{ab}}        \}_{k_{ac}};$\\
\\
$Access(\alpha,m)=\{\{k_{ac}^{-1},k_{ab}^{-1}\}, \{k_{ac}^{-1}\},\{k_{ac}^{-1},k_{ab}^{-1},k_{ef}^{-1}\}\}$.
\begin{comment}
\begin{tabular}{lll}
  $Access(\alpha,\{ A.D.\alpha \}_{k_{ab}})$&$=$& $k_{ab}^{-1} \otimes (Access(\alpha,A) \cup $\\
  &&$ Access(\alpha,D) \cup$\\
  && $Access(\alpha,\alpha))$\\
  &$=$&$k_{ab}^{-1} \otimes (\emptyset \cup \emptyset \cup \{\emptyset\})$\\
  &$=$&$\{\{k_{ab}^{-1}\}\}$\\
  &&\\
\end{tabular}

\begin{tabular}{lll}
  $Access(\alpha,\{C.\alpha\}_{k_{ef}}))$& $=$ &$k_{ef}^{-1} \otimes Access(\alpha,C)\cup Access(\alpha,\alpha)$\\
                                         & $=$ &$k_{ef}^{-1} \otimes (\emptyset \cup \{\emptyset\})$\\
                                         & $=$ &$\{\{k_{ef}^{-1}\}\}$\\

  &&\\
\end{tabular}

\begin{tabular}{lll}
  $ Access(\alpha,\{ A.E.\{C.\alpha\}_{k_{ef}}\}_{k_{ab}})$ & $=$ & $k_{ab}^{-1} \otimes Access(\alpha,A.E.\{C.\alpha\}_{k_{ef}})$\\
  &$=$&$k_{ab}^{-1} \otimes (Access(\alpha,A)\cup $\\
  &&$Access(\alpha,E)\cup $\\
  &&$Access(\alpha,\{C.\alpha\}_{k_{ef}}))$\\
    &$=$&$k_{ab}^{-1} \otimes (\emptyset \cup \emptyset\cup Access(\alpha,\{C.\alpha\}_{k_{ef}}))$\\
    &$=$&$k_{ab}^{-1} \otimes (Access(\alpha,\{C.\alpha\}_{k_{ef}}))$\\
    &$=$&$k_{ab}^{-1} \otimes \{\{k_{ef}^{-1}\}\}$\\
    &$=$&$\{\{k_{ab}^{-1},k_{ef}^{-1}\}\}$\\
  &&\\
\end{tabular}

\begin{tabular}{lll}
  $Access(\alpha,m)$ & $=$ & $k_{ac}^{-1} \otimes (Access(\alpha,\{ A.D.\alpha \}_{k_{ab}}.\alpha.\{ A.E.\{C.\alpha\}_{k_{ef}} \}_{k_{ab}}))$ \\
   & $=$ & $k_{ac}^{-1} \otimes (Access(\alpha,\{ A.D.\alpha \}_{k_{ab}})\cup$\\
   &&$ Access(\alpha,\alpha)\cup$\\
   &&$ Access(\alpha,\{ A.E.\{C.\alpha\}_{k_{ef}}\}_{k_{ab}}))$ \\
   &$=$&$k_{ac}^{-1} \otimes (\{\{k_{ab}^{-1}\}\} \cup \{\emptyset\}\cup \{\{k_{ab}^{-1},k_{ef}^{-1}\}\})$\\
   &$=$&$\{\{k_{ac}^{-1},k_{ab}^{-1}\}\} \cup \{\{k_{ac}^{-1}\}\} \cup \{\{k_{ac}^{-1},k_{ab}^{-1},k_{ef}^{-1}\}\}$\\
   &$=$&$\{\{k_{ac}^{-1},k_{ab}^{-1}\}, \{k_{ac}^{-1}\},\{k_{ac}^{-1},k_{ab}^{-1},k_{ef}^{-1}\}\}$\\
 %%  &$=$&$\{\{k_{AC},k_{AB}\}, \{k_{AC}\},\{k_{AC},k_{AB},k_{EF}\}\}$\\

\end{tabular}
\end{comment}
\end{exemple}

\begin{defini}(Well-protected message)\label{bienprotege}
$ $\\
\\
Let ${\mathcal{C}}$ be a context of verification and $m\in{\mathcal{M}}$ and $M \subseteq {\mathcal{M}}$.
\\
Let $\alpha \in {\mathcal{A}}(m)$ such that $\ulcorner \alpha \urcorner \sqsupset \bot$.\\
\\
We say that $\alpha$ is well-protected in $m$ if:
\[
\forall \beta \in Access(\alpha,m).\ulcorner \beta \urcorner \sqsupseteq \ulcorner \alpha \urcorner
\]
We say that $\alpha$ is well-protected in $M$ if:
\[
\forall m\in M.\alpha \mbox{ is well-protected in } m
\]
We say that $m$ is well-protected in ${\mathcal{C}}$ if:
\[\forall \alpha \in {\mathcal{A}}(m). \alpha \mbox{ is well-protected in } m\]
We say that $M$ is well-protected in ${\mathcal{C}}$ if:

\[\forall m \in M. m \mbox{ is well-protected in }{\mathcal{C}}.\]

\end{defini}
Informally, a well-protected message is a message such that every atom $\alpha$ in it such that $\ulcorner \alpha \urcorner \sqsupset \bot$ is encrypted by at least one key $k$ such that  $\ulcorner k^{-1} \urcorner \sqsupseteq \ulcorner \alpha \urcorner$ after elimination of unnecessary keys by the normal form.

\begin{defini}($Clear$)\label{clearmProofs}
$ $\\
Let $m\in {\mathcal{M}}$ and $M\subset {\mathcal{M}}$.
$$Clear(m)=\{\alpha \in {\mathcal{A}}(m). \mbox{     } \emptyset \in Access(\alpha,m)\}$$
We extend this definition to sets as follows:
%%Cette définition is prolongée sur les ensembles as follows:\\
$$Clear(M)={\underset {m\in M}{\cup}}Clear(m)$$

\end{defini}
$ $\\
Informally, $Clear(m)$ is the set of all atoms that appear in clear in $m$ after elimination of unnecessary keys by the normal form.

\begin{cor}\label{prepositionatomique}
$ $\\
Let  ${\mathcal{C}}=\langle{\mathcal{M}},\xi,\models,{\mathcal{K}},{\mathcal{L}}^\sqsupseteq,\ulcorner .\urcorner\rangle$ be a context  of verification.\\
Let $m$ a well-protected message in ${\mathcal{M}}$.\\
Let $\alpha \in {\mathcal{A}}(m)$.\\
We have:
\[\alpha \in Clear(m) \Rightarrow \ulcorner \alpha \urcorner=\bot\]
\end{cor}
$ $\\
See the proof \ref{PR21}.\\
\begin{preuve}\label{PR21}
$ $\\
Let $\alpha \in {\mathcal{A}}(m)$.\\
\\
$m$ is well-protected then from the definition \ref{bienprotege} we have:
\begin{equation}
\mbox{ if }\ulcorner \alpha \urcorner \sqsupset \bot \mbox{ then }  \forall \beta \in Access(\alpha,m).\ulcorner \beta \urcorner \sqsupseteq \ulcorner \alpha \urcorner \label{preuveprepositionatomique1}
\end{equation}
For $\alpha \in Clear(m)$, we have from the definition \ref{clearmProofs}:
\begin{equation}
\emptyset \in Access(\alpha,m)\label{preuveprepositionatomique2}
\end{equation}
Let $\beta=\emptyset$, then we have: \begin{equation}
\not\exists k \in \beta. \ulcorner k\urcorner\sqsupseteq \ulcorner \alpha \urcorner \label{preuveprepositionatomique21}
\end{equation}
But \ref{preuveprepositionatomique21} is the definition of:
\begin{equation}
 \ulcorner \beta \urcorner \not\sqsupseteq \ulcorner \alpha \urcorner \label{preuveprepositionatomique2199}
\end{equation}
Then from \ref{preuveprepositionatomique2} and \ref{preuveprepositionatomique2199}:
\begin{equation}
\exists \beta \in Access(\alpha,m). \ulcorner \beta \urcorner \not \sqsupseteq \ulcorner \alpha \urcorner \label{preuveprepositionatomique3}
\end{equation}
From \ref{preuveprepositionatomique3} and \ref{preuveprepositionatomique1} we have:
\begin{equation}
\ulcorner \alpha \urcorner \not \sqsupset \bot
\label{preuveprepositionatomique4}
\end{equation}
Or else:
\begin{equation}
\ulcorner \alpha \urcorner=\bot \label{preuveprepositionatomique5}
\end{equation}
\\
\end{preuve}

\begin{lem}{}\label{lemConservationBPMouchArticle}
$ $\\
\\
Let $M$ be a set of well-protected messages in ${\mathcal{M}}$ and ${\mathcal{C}}$ be a context of verification. We have:
\[
M\models_{\mathcal{C}} m \Rightarrow \forall \alpha \in {\mathcal{A}}(m).(\alpha \mbox{ is well-protected in }m) \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner)
\]
\end{lem}
$ $\\
See the proof \ref{Pr22Proofs}


\begin{preuve}\label{Pr22Proofs}
$ $\\
\\
We suppose that an intruder has the three following rules of building messages:\\

  $(int):$ $\frac{\square}{M\models_{\mathcal{C}} m}[m\in M\cup K(I)] $\\

  $(op):$$\frac{M\models_{\mathcal{C}} m_1,..., M\models_{\mathcal{C}} m_n }{M\models_{\mathcal{C}} f(m_1,...,m_n)}[f\in \Sigma]$\\

  $(eq):$$\frac{M\cup K(I) \models_{\mathcal{C}} m', m'=_{\mathcal{C}} m}{M\cup K(I) \models_{\mathcal{C}} m}$\\
\\
Let's run the proof by induction on the size of the tree of building $m$.\\
%%\begin{itemize}
\begin{itemize}

\item[$\bullet$]For $|M\models_{\mathcal{C}} m|=1$.\\
\\
In this case, the only applicable rule is $(int)$. We have two cases:\\

* $m \in M$,\\

In this case, and since $M$ is a well-protected set of messages, we have directly: $m$ is well-protected.\\
\\
Then, from the definition \ref{bienprotege} we have: \begin{equation}  \forall \alpha \in {\mathcal{A}}(m). \alpha \mbox{ is well-protected in } m \label{preuvelematomique2MODIF} \end{equation}

* $m \in K(I)$, \\

In this case, $m$ is atomic because $K(I)$ is by assumption an atomic set.\\
\\
Then:
\begin{equation} \forall \alpha \in {\mathcal{A}}(m).\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner \label{preuvelematomique3MODIF} \end{equation}
\\
From \ref{preuvelematomique2MODIF} and \ref{preuvelematomique3MODIF} we have:
\begin{equation} \forall \alpha \in {\mathcal{A}}(m).(\alpha \mbox{ is well-protected in }m) \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{preuvelematomique3MODIFBIS} \end{equation}
\end{itemize}
Let's assume for all $p \leq n$, for all $M\subseteq {\mathcal{M}}$ and $m\in {\mathcal{M}}$ such that $|M\models_{\mathcal{C}} m|=p$, we have:
\begin{equation}\forall \alpha \in {\mathcal{A}}(m).(\alpha \mbox{ is well-protected in }m) \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{preuvelematomique4MODIF} \end{equation}
Let's prove this result for $p=n+1$.\\
\begin{itemize}
\item[$\bullet$] For $|M\models_{\mathcal{C}} m|=n+1$
\\
    \begin{itemize}
    \item[$\bullet$] If the used rule  is $(op):$$\frac{M\models_{\mathcal{C}} m_1,..., M\models_{\mathcal{C}} m_n }{M\models_{\mathcal{C}} f(m_1,...,m_n)}[f\in \Sigma]$ with:

    \begin{equation} f(m_1,...,m_n)=m \end{equation}

    Let $\alpha \in {\mathcal{A}}(m)$ such that $\alpha \sqsupset \bot$.\\
    \\
    We have two cases:\\
    \\
    \underline{\textbf{First Case:}} $f \in \overline{{\mathcal{E}}}_{\mathcal{C}}$\\
    \\
    In this case, and since the application $Access$ in not sensitive to non-encryption functions, we have:
   %% Dans ce cas, and puisque l'application $Access$ is par construction insensible aux non-encryptions, we have:
    \begin{equation}
    Access(\alpha,m) \subseteq Access(\alpha,M)\label{preuvelematomique4MODIF2}
    \end{equation}
    Let $\beta \in Access(\alpha,m)$.\\
    \\
    From \ref{preuvelematomique4MODIF2} we have:
    \begin{equation}
    \beta \in Access(\alpha,M)\label{preuvelematomique4MODIF3}
    \end{equation}
    But $M$ is a set of well-protected messages in ${\mathcal{C}}$, then:
    \begin{equation}
    \ulcorner \beta \urcorner \sqsupseteq \ulcorner \alpha \urcorner\label{preuvelematomique4MODIF4}
    \end{equation}
    The result \ref{preuvelematomique4MODIF4} stands $\forall \beta \in Access(\alpha,m)$, so we have:
    \begin{equation}
    \forall \beta \in Access(\alpha,m).\ulcorner \beta \urcorner \sqsupseteq \ulcorner \alpha \urcorner\label{preuvelematomique4MODIF5}
    \end{equation}
    From \ref{preuvelematomique4MODIF5} and the definition \ref{bienprotege} we have:
    \begin{equation}
    \alpha \mbox{ is well-protected in }m\label{preuvelematomique4MODIF6}
    \end{equation}
    \underline{\textbf{Second case:}} $f_k \in {\mathcal{E}}_{\mathcal{C}}$\\
    \\
    In this case, we have two sub-cases:\\
     \begin{enumerate}
       \item First sub-case:
           \begin{equation}
            \forall \beta \in Access(\alpha,m).\ulcorner \beta \urcorner \sqsupseteq \ulcorner \alpha \urcorner\label{preuvelematomique4MODIF7}
           \end{equation}
          In this sub-case, from \ref{preuvelematomique4MODIF7} and the definition \ref{bienprotege} we have:
           \begin{equation}
            \alpha \mbox{ is well-protected in }m\label{preuvelematomique4MODIF9}
           \end{equation}
       \item Second sub-case:
           \begin{equation}
            \exists \beta \in Access(\alpha,m).\ulcorner \beta \urcorner \not\sqsupseteq \ulcorner \alpha \urcorner\label{preuvelematomique4MODIF10}
           \end{equation}
           In this sub-case, $f_k$ is necessary a decryption that decreases an element of  $ Access(\alpha,M)$ from the value  $(\{k^{-1}\}\cup\beta)$ in $M$ to the value $\beta$ in $m$, with $(\{k^{-1}\}\cup\beta)\in Access(\alpha,M)$.\\

           Since $M$ is a well-protected set, then:
           \begin{equation}
            \ulcorner \{k^{-1}\}\cup\beta \urcorner \sqsupseteq \ulcorner \alpha \urcorner\label{preuvelematomique4MODIF11}
           \end{equation}
           From \ref{preuvelematomique4MODIF10} and \ref{preuvelematomique4MODIF11} we have:
           \begin{equation}
            \ulcorner k^{-1} \urcorner \sqsupseteq \ulcorner \alpha \urcorner\label{preuvelematomique4MODIF12}
           \end{equation}
           Since $f_k \in {\mathcal{E}}_{\mathcal{C}}$ (encryption), so the intruder should have retieved the key  $(\{k^{-1}\}$ in a previous step of the induction. i.e:
           \begin{equation}
           \exists p \leq n \mbox{ such that }|M\models_{\mathcal{C}} k^{-1}|=p.
           \label{preuvelematomique4MODIF13}
           \end{equation}
           From \ref{preuvelematomique4MODIF13} and from the assumption of induction in \ref{preuvelematomique4MODIF} we have:
           \begin{equation}(k^{-1} \mbox{ is well-protected in }k^{-1}) \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner k^{-1} \urcorner) \label{preuvelematomique4MODIF14} \end{equation}
           But $k^{-1} \mbox{ is not well-protected in }k^{-1}$ since $k^{-1} \mbox{ is clear in }k^{-1}$, so we have from \ref{preuvelematomique4MODIF14}:
           \begin{equation}\ulcorner K(I) \urcorner \sqsupseteq \ulcorner k^{-1} \urcorner \label{preuvelematomique4MODIF15} \end{equation}
           From \ref{preuvelematomique4MODIF12} and \ref{preuvelematomique4MODIF15} we have:
           \begin{equation}\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner
           \label{preuvelematomique4MODIF16} \end{equation}
     \end{enumerate}

    \item[$\bullet$] If the used rule is $(eq):$$\frac{M\cup K(I) \models_{\mathcal{C}} m', m'=_{\mathcal{C}} m}{M\cup K(I) \models_{\mathcal{C}} m}$\\
\\
Since $ m'=_{\mathcal{C}} m$ then:
    \begin{equation}
     m'_\Downarrow= m_\Downarrow \label{preuvelematomique5}\\
    \end{equation}

    Let $\alpha\in {\mathcal{A}}(m')$ such that $\alpha \sqsupset \bot$.\\
    \\
    From the definition of the application $Access$:\\
    \begin{equation}
    Access(\alpha, m')= Access(\alpha, m'_\Downarrow) \label{preuvelematomique6}\\
    \end{equation}
    \[\mbox{ and }
    \]
    \begin{equation}
    Access(\alpha, m)= Access(\alpha, m_\Downarrow) \label{preuvelematomique6MODIF}\\
    \end{equation}
    Since $m'$ comes from a previous step of the induction and since $M$ is a well-protected set ${\mathcal{C}}$, then from the assumption of induction in \ref{preuvelematomique4MODIF} we have:\\
    \begin{equation}(\alpha \mbox{ is well-protected in }m') \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{preuvelematomique4MODIF17} \end{equation}
    From the definition \ref{bienprotege} and \ref{preuvelematomique4MODIF17} we have:
    \begin{equation}(\forall \beta \in Access(\alpha,m').\ulcorner \beta \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{preuvelematomique4MODIF19} \end{equation}
    From \ref{preuvelematomique5}, \ref{preuvelematomique6}, \ref{preuvelematomique6MODIF} and \ref{preuvelematomique4MODIF19} we have:
    \begin{equation}(\forall \beta \in Access(\alpha,m).\ulcorner \beta \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{preuvelematomique4MODIF20} \end{equation}
    From the definition \ref{bienprotege} and \ref{preuvelematomique4MODIF20} we have:
    \begin{equation}(\alpha \mbox{ is well-protected in }m) \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{preuvelematomique4MODIF21} \end{equation}
  \end{itemize}

    From \ref{preuvelematomique4MODIF6}, \ref{preuvelematomique4MODIF9}, \ref{preuvelematomique4MODIF16} and \ref{preuvelematomique4MODIF21} we have: $\mbox{for } |M\models_{\mathcal{C}} m|=n+1$:\\
    \begin{equation}\forall \alpha \in {\mathcal{A}}(m).(\alpha \mbox{ is well-protected in }m) \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{preuvelematomique11} \end{equation}

\end{itemize}
$ $\\
From \ref{preuvelematomique4MODIF} and \ref{preuvelematomique11} we deduce that: for all $M\models_{\mathcal{C}} m $, we have:
\\
\begin{equation}\forall \alpha \in {\mathcal{A}}(m).(\alpha \mbox{ is well-protected in }m) \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner)\end{equation}
%%\end{itemize}
\end{preuve}

The lemma \ref{lemConservationBPMouchArticle} states that from a set of well-protected messages, all atomic messages beyond the knowledge of the intruder (i.e. $\ulcorner K(I) \urcorner \not \sqsupseteq \ulcorner \alpha \urcorner$) remain well-protected in any message that the intruder could infer. In fact, since we operate on well-protected messages, every atom such that  $\ulcorner \alpha  \urcorner \not \sqsupset \bot$ is encrypted by at least one key $k$ such that $\ulcorner k^{-1} \urcorner \sqsupseteq \ulcorner \alpha \urcorner$. So the intruder must retrieve $k^{-1}$ before she sees $\alpha$ not well-protected in any message. Yet, the key $k^{-1}$  is, in its turn, encrypted by at least one key $k'$ such that $\ulcorner k'^{-1} \urcorner \sqsupseteq \ulcorner k^{-1} \urcorner$ since we operate on well-protected messages. The proof is then run by induction on the encryption keys.

\begin{lem}(Lemma of non-disclosure of atomic secrets in well-protected messages)\label{lematomiqueProofs}
\\
Let $M$ be a set of well-protected messages in ${\mathcal{M}}$ and $\alpha$ an atomic message in $M$. \\
We have:
\[M\models_{\mathcal{C}} \alpha \Rightarrow \ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner.\]
\end{lem}
$ $\\
See the proof \ref{PR23}

\begin{preuve}\label{PR23}
$ $\\
\\
From the lemma \ref{lemConservationBPMouchArticle}, we have $M\models_{\mathcal{C}} \alpha$ then:
\begin{equation}(\alpha \mbox{ is well-protected in }\alpha) \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner)\label{preuveCons1}\end{equation}
But $\alpha \mbox{ is not well-protected in }\alpha$, then we have:
\begin{equation}\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner\label{preuveCons2}\end{equation}
\end{preuve}



The lemma \ref{lematomiqueProofs} expresses an important result. It states that from a set of well-protected messages the intruder can never deduce a secret that she is not initially allowed to know when using her knowledge in a context of verification only.  We assume throughout the rest of this work that all protocols we analyze operate over a space of well-protected messages which is easy to verify.

%% When a message has a unique form (i.e. when we have an empty equational theory), it is easy to verify if a message is well-protected or not. However,  with a non-empty equational theory~\cite{cortier9900,cortier1971,cortier9901}, we need to check all the forms that are equivalent to the message provided within the specification of the protocol. To make the analysis simple, we assume that we can extract from our equational theory a  convergent rewriting system~\cite{FranzRewriting,Rewriting,LoulergueRewriting} oriented in such way that the normal form is the one having the smallest set of encryption keys (e.g. $e(k,d(k^{-1},m))\rightarrow m$). The same assumption had been made in the definition \ref{bienprotegeArt}. This kind of orientation of rewriting systems poses no problem in the most of equational theories of the intruder in the litterature.%% and the most reduced one. %%We call this form the canonical form and we denote it by $m_{\Downarrow}$. %%We assume throughout the rest of this work that all protocols we analyze operate over a space of well-protected messages where all messages are normalized that way.

\section{Intermediate results and proofs for Reliability of selections inside the external key}


\begin{defini}(Well-formed selection)\label{selecBFProofs}
$ $\\
Let $M,M_1,M_2\subseteq {\mathcal{M}}$ such that $M, M_1$ and $M_2$ are well-protected and ${\mathcal{C}}$ be a context of verification.\\
Let $S: {\mathcal{A}}\times {\mathcal{M}}\longmapsto{2^{\mathcal{A}}}$ be a selection.\\
We say that $S$ is well-formed in ${\mathcal{C}}$ if:
\[
\left\{
    \begin{array}{lll}
         S(\alpha,\{\alpha\})&=&{\mathcal{A}},\\
         S(\alpha, {M}_1 \cup {M}_2)&=&S(\alpha, {M}_1)\cup S(\alpha,{M}_2),\\
         S(\alpha,{M})&=&\emptyset  \mbox{, if } \alpha \notin {\mathcal{A}}({M})\\
    \end{array}
\right.
\]
\end{defini}

For an atom $\alpha$ in a set of messages $M$, a well-formed selection returns all the atoms in ${\mathcal{M}}$ if $M=\{\alpha\}$. It returns for it in the union of two sets of messages, the union of the two selections performed in each set separately. It returns the empty set if the atom does not appear in $M$.
\normalsize

\begin{defini}(Full-invariant-by-intruder selection)\label{DefFnInterIsotropProofs}
$ $\\
Let $M\subseteq {\mathcal{M}}$ such that $M$ is well-protected and ${\mathcal{C}}$ be a context of verification.\\
Let $S: {\mathcal{A}}\times {\mathcal{M}}\longmapsto{2^{\mathcal{A}}}$ be a selection.\\
We say that $S$ is full-invariant-by-intruder in ${\mathcal{C}}$ if:\\
$\forall m \in {\mathcal{M}},$ we have:
\[
M \models_{\mathcal{C}} m\Rightarrow  \forall \alpha \in {\mathcal{A}}(m).(S(\alpha,m) \subseteq S(\alpha,M))\vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner)
\]

\end{defini}

\begin{defini}(Reliable selection)\label{selecreliableProofs}
$ $\\
Let $S: {\mathcal{A}}\times {\mathcal{M}}\longmapsto{2^{\mathcal{A}}}$ be a selection and ${\mathcal{C}}$ be a context of verification.
\[S  \mbox { is }{\mathcal{C}}\mbox{-reliable } \mbox{if}  \mbox{ } S \mbox{ is well-formed }  \mbox{and }  S \mbox{ is full-invariant-by-intruder in } {\mathcal{C}}.\]
\end{defini}

\begin{defini}($S_{Gen}^{EK}$: selection inside the protection of an external key)\label{SGENProofs}
$ $\\
We denote by $S_{Gen}^{EK}$ the class of all selections $S$ that meet the following conditions:\\
\\
$
\bullet ~S(\alpha,\alpha)={\mathcal{A}};$\begin{equation}\label{PremierelemInt1DefSgen1Proofs}\end{equation}
$\bullet ~S(\alpha,m)=\emptyset \mbox{,   if   } \alpha \not \in {\mathcal{A}}(m);$ \begin{equation}\label{PremierelemInt1DefSgen2Proofs}\end{equation}
$\bullet ~\forall \alpha \in {\mathcal{A}}(m),  \mbox { where } m=f_k(m_1, ..., m_n):$
\begin{equation}S(\alpha,m)  \subseteq (\underset{1\leq i \leq n}{\cup} {\mathcal{A}}(m_i){\cup} \{k^{-1}\}\backslash\{\alpha\})  \mbox{    if } f_k \in {\mathcal{E}}_{\mathcal{C}} \mbox{ and }\ulcorner {k^{-1}}\urcorner \sqsupseteq \ulcorner \alpha \urcorner \mbox{ and } m=m_\Downarrow\mbox{ } \label{PremierelemInt1DefSgen2222Proofs}\end{equation}
$\bullet ~\forall \alpha \in {\mathcal{A}}(m), \mbox { where } m=f(m_1, ..., m_n):$
\begin{equation}
%\left\{
S(\alpha,m)=    \begin{cases}
        \underset{1\leq i \leq n}{\cup} S(\alpha,m_i)& \mbox{if }  f_k \in {\mathcal{E}}_{\mathcal{C}} \mbox{ and } \ulcorner {k^{-1}}\urcorner \not \sqsupseteq \ulcorner \alpha \urcorner \mbox{ and } m=m_\Downarrow\mbox{ }  \mbox{    (a)}\\
        \underset{1\leq i \leq n}{\cup} S(\alpha,m_i) & \mbox{if } f\in \overline{{\mathcal{E}}}_{\mathcal{C}} \mbox{ and } m=m_\Downarrow \mbox{ }  \mbox{   (b)} \\
        S(\alpha,m_\Downarrow) &  \mbox{if } m\not=m_\Downarrow \mbox{   (c)}
    \end{cases}
%\right.
\label{PremierelemInt1DefSgen3Proofs}
\end{equation}
%%and extented to sets as follows:
$\bullet ~S(\alpha,\{m\}\cup M)=S(\alpha,m) \cup S(\alpha,M)$\begin{equation}
 \label{PremierelemInt1DefSgen4Proofs}
\end {equation}
%%We denote by $S_{Gen}^{EK}$ the class of all selections inside the protection of an external key.$\Box$
\end{defini}

\begin{pre}\label{PremierelemInt1Proofs}
$ $\\
\\
Let  ${\mathcal{C}}=\langle{\mathcal{M}},\xi,\models,{\mathcal{K}},{\mathcal{L}}^\sqsupseteq,\ulcorner .\urcorner\rangle$ be a context  of verification.\\
Let $S$ be an instance of $S_{Gen}^{EK}$.
\\
Let's have a rewriting system $\rightarrow_{\xi}$ such that $\forall m \in {\mathcal{M}},\forall \alpha \in {\mathcal{A}}(m) \wedge \alpha \not \in Clear(m),$ we have: \begin{equation} \forall l \rightarrow r \in \rightarrow_{\xi},S(\alpha,r) \subseteq S(\alpha,l)\label{eqRewSystSFIBIMouchArtProofs} \end{equation}
We have:
%% $S$ définie en \ref{PremierelemInt1Proofs} is full-invariant-by-intruder in ${\mathcal{C}}$.\\
\center{$S$   is full-invariant-by-intruder in ${\mathcal{C}}$.}\\
\end{pre}
See the proof \ref{PR24}.
\begin{remarque}\label{RemRWSYSSFIBIProofs}
$ $\\
\\
The condition on the rewriting system $\rightarrow_{\xi}$ given by the equation \ref{eqRewSystSFIBIMouchArtProofs} in the proposition \ref{PremierelemInt1Proofs} is introduced to make sure that the selection in the normal form is the smallest among all forms of a given message. This prevents the selection $S$ to select atoms that are inserted maliciously by the intruder by manipulating the equational theory. Hence, we are sure that all selected atoms by $S$ are honest and do not come by an intruder manipulation of the message. For example, let $m=\{\alpha.D\}_{k_{ab}}$ be a message in a homomorphic cryptography (i.e. $\{\alpha.D\}_{k_{ab}}=\{\alpha\}_{k_{ab}}.\{D\}_{k_{ab}}$). In the form $\{\alpha.D\}_{k_{ab}}$, the selection $S(\alpha,\{\alpha.D\}_{k_{ab}})$ may select $D$, but in the form $\{\alpha\}_{k_{ab}}.\{D\}_{k_{ab}}$, the selection $S(\alpha,\{\alpha\}_{k_{ab}}.\{D\}_{k_{ab}})$ may not. Then, we must make sure that the rewriting system $\rightarrow_{\xi}$ we are using is oriented in such way that it chooses the form $\{\alpha\}_{k_{ab}}.\{D\}_{k_{ab}}$ rather than the form $\{\alpha.D\}_{k_{ab}}$ because there is no guarantee that $D$ is a honest neighbor and that it had not been inserted maliciously by the intruder using the homomorphic property in the theory. We assume that the rewriting system we are using meets this condition.
\end{remarque}


\begin{preuve}\label{PR24}
$ $\\
\\
Let $S$ be an instance of $S_{Gen}^{EK}$.\\
\\
We suppose that the intruder has the following rules:\\
\\
  $(int):$ $\frac{\square}{M\models_{\mathcal{C}} m}[m\in M\cup K(I)] $\\
\\
  $(op):$$\frac{M\models_{\mathcal{C}} m_1,..., M\models_{\mathcal{C}} m_n }{M\models_{\mathcal{C}} f(m_1,...,m_n)}[f\in \Sigma]$\\
\\
 $(eq):$$\frac{M\models_{\mathcal{C}} m', m'=_{\mathcal{C}} m}{M\models_{\mathcal{C}} m}$\\
\\
Let's run the proof by induction on the size of the tree of building $m$.\\
%%\begin{itemize}
%%\item[$\bullet$]



\begin{itemize}

\item[$\bullet$] For $|M\models_{\mathcal{C}} m|=1$.\\

In this case, the only applicable rule is $(int)$.\\
\\
We have two cases:\\
\\
* $m\in M$, \\
   Then: $\{m\}\cup M=M$\\
   Then: $S(\alpha,\{m\}\cup M)=S(\alpha,\{m\}) \cup S(\alpha,M)=S(\alpha,M)$\\
   Then:
   \begin{equation}S(\alpha,\{m\}) \subseteq S(\alpha,M) \label{premierePreuvelemInt1} \end{equation}\
\\
* $m \in K(I)$,\\ 
In this case, $m=\alpha$ must be atomic since $K(I)$ is by assumption a set of atomic messages.\\
We have then:
\begin{equation}\ulcorner K(I)\urcorner \sqsupseteq \ulcorner\alpha \urcorner \label{premierePreuvelemInt2} \end{equation}\
From \ref{premierePreuvelemInt1} and \ref{premierePreuvelemInt2} we conclude that for $|M\models_{\mathcal{C}} m|=1$:
\begin{equation} M\models_{\mathcal{C}} m\Rightarrow \forall \alpha \in {\mathcal{A}}(m).(S(\alpha,m) \subseteq S(\alpha,M))\vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \end{equation}\
\end{itemize}
We assume that for $1 \leq i \leq n$, for all well-protected $M$ and $m$ such that $|M\models_{\mathcal{C}} m|=p$, we have:\\
   \begin{equation} M\models_{\mathcal{C}} m \Rightarrow \forall \alpha \in {\mathcal{A}}(m).(S(\alpha,m) \subseteq S(\alpha,M))\vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{premierePreuvelemInt3} \end{equation}
Let's prove this result for $|M\models_{\mathcal{C}} m|=n+1$.\\
\begin{itemize}
\item[$\bullet$]For $|M\models_{\mathcal{C}} m|=n+1$\\
    \begin{itemize}
    \item[$\bullet$] If the used rule is $(op)$:\\
\\
    Let $m=f_k(m_1,...,m_n)$ with $ M\models_{\mathcal{C}} m_i$ for $i\in [1..n]$.\\
    \begin{itemize}
    \item[$\bullet$] If $\alpha \in Clear(M)$\\
    \\
    Since $M$ is well-protected, we have from the corollary \ref{prepositionatomique}:
       \begin{equation}\ulcorner \alpha \urcorner=\bot \label{premierePreuvelemInt4} \end{equation}

    Then, \begin{equation}\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner \label{premierePreuvelemInt5} \end{equation}

    \item[$\bullet$] If $\alpha \not \in Clear(M)$\\
    \\
    In this case, from the definition of $Clear(M)$ we have:

    \begin{equation}
    \forall \beta \in Access(\alpha,M). \beta \neq \emptyset \label{premierePreuvelemInt5bis}
    \end{equation}

    From the definition of $S$, we have four sub-cases:\\

    1-$f_k \in {\mathcal{E}}_{\mathcal{C}}\mbox{ and }\ulcorner {k^{-1}}\urcorner \sqsupseteq \ulcorner \alpha \urcorner \mbox{ and } f_k(m_1, ..., m_n)=f_k(m_1, ..., m_n)_\Downarrow$\\

    In this sub-case:

    \begin{equation}S(\alpha,f_k(m_1, ..., m_n)) \subseteq \underset{1\leq i \leq n}{\cup}{\mathcal{A}}(m_i) {\cup}\{k^{-1}\}\backslash\{\alpha\} \label{premierePreuvelemInt6} \end{equation}

   We have by definition of $S$ in this case:

    \begin{equation}\ulcorner k^{-1} \urcorner \sqsupseteq \ulcorner \alpha \urcorner \label{premierePreuvelemInt8} \end{equation}

From \ref{premierePreuvelemInt6}, $S$ selects its items in a section encrypted by the key $k$. As seen in the remark \ref{RemRWSYSSFIBIProofs}, the condition on the rewriting system \ref{eqRewSystSFIBIMouchArtProofs} in the proposition \ref{PremierelemInt1Proofs} makes sure that atoms in this section could not be altered by using the equational theory. So, before altering this section, it is necessary for the intruder to have found the key $\{k^{-1}\}$ in a previous step of the induction, i.e.:

    \begin{equation}\exists p \leq n, |M\models_{\mathcal{C}} k^{-1}|=p \label{premierePreuvelemInt8biss} \end{equation}

   Since $k^{-1}$ is atomic and $M$ is well-protected, then from the lemma \ref{lematomique} and  \ref{premierePreuvelemInt8biss} we have:
    \begin{equation}\ulcorner K(I)\urcorner \sqsupseteq \ulcorner k^{-1} \urcorner \label{premierePreuvelemInt9} \end{equation}

    From \ref{premierePreuvelemInt8} and \ref{premierePreuvelemInt9} we have:

    \begin{equation}\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner \label{premierePreuvelemInt10} \end{equation}

    2-$f_k \in {\mathcal{E}}_{\mathcal{C}} \mbox{ and } \ulcorner {k^{-1}}\urcorner \not \sqsupseteq \ulcorner \alpha \urcorner \mbox{ and } f_k(m_1, ..., m_n)=f_k(m_1, ..., m_n)_\Downarrow$\\

    In this sub-case we have:

    \begin{equation}S(\alpha,f_k(m_1, ..., m_n)) = \underset{1\leq i \leq n}{\cup} S(\alpha,m_i) \label{premierePreuvelemInt11} \end{equation}

    Since each message $m_i$ $(1\leq i \leq n)$ comes from a previous step of the induction $(|M\models_{\mathcal{C}} m_i|\leq n)$, and from the assumption of the induction in \ref{premierePreuvelemInt3} we have for all $m_i\in \{m_1,...,m_n\}$ and for all $\alpha\in {\mathcal{A}}(m_i)\mbox{ such that }\ulcorner K(I) \urcorner\not \sqsupseteq \ulcorner\alpha\urcorner$:
    \begin{equation}S(\alpha,m_i) \subseteq S(\alpha,M) \label{eqjdida2MOD}\end{equation}

    From \ref{eqjdida2MOD} we have:
    \begin{equation}\underset{1\leq i \leq n}{\cup}S(\alpha,m_i) \subseteq \underset{1\leq i \leq n}{\cup}S(\alpha,M) \label{eqjdida3MOD}\end{equation}
    Or else:
    \begin{equation}\underset{1\leq i \leq n}{\cup}S(\alpha,m_i) \subseteq S(\alpha,M) \label{eqjdida4MOD}\end{equation}
    From \ref{premierePreuvelemInt11} and \ref{eqjdida4MOD} we have:\\
    \begin{equation}S(\alpha,f_k(m_1,...,m_n))\subseteq S(\alpha,M) \label{eqjdida5MOD}\end{equation}
    From \ref{eqjdida2MOD} and \ref{eqjdida5MOD}:
    \begin{equation}S(\alpha,f_k(m_1,...,m_n))\subseteq S(\alpha,M) \vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner\alpha\urcorner) \label{premierePreuvelemInt14GR} \end{equation}
    The result \ref{premierePreuvelemInt14GR} stands for all $\alpha\in{\mathcal{A}}(m)$ where $m=f_k(m_1, ..., m_n)$, then:
     \begin{equation}\forall \alpha \in {\mathcal{A}}(m).(S(\alpha,m) \subseteq S(\alpha,M))\vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{premierePreuvelemInt14} \end{equation}

    3-$f\in \overline{{\mathcal{E}}}_{\mathcal{C}} \mbox{ and } f(m_1, ..., m_n)=f(m_1, ..., m_n)_\Downarrow$,\\

   This sub-case joins the sub-case 2. Then, we have directly:
    \begin{equation}\forall \alpha \in {\mathcal{A}}(m).(S(\alpha,m) \subseteq S(\alpha,M))\vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{premierePreuvelemInt16} \end{equation}

    4-$f(m_1, ..., m_n)\not=f(m_1, ..., m_n)_\Downarrow$,\\

   In this subcase, we normalize only. No selection is performed.\\

    \end{itemize}
    From \ref{premierePreuvelemInt5}, \ref{premierePreuvelemInt10}, \ref{premierePreuvelemInt14} and \ref{premierePreuvelemInt16} we have:
\begin{equation}\forall \alpha \in {\mathcal{A}}(m).(S(\alpha,m) \subseteq S(\alpha,M))\vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{premierePreuvelemInt17} \end{equation}




    \item[$\bullet$] If the used rule is $(eq)$:\\

    We have:

    \begin{equation}M\models_{\mathcal{C}} m', m'=_{\mathcal{C}} m \label{premierePreuvelemInt18} \end{equation}

    From \ref{premierePreuvelemInt18} and from the uniqueness of the normal form we have:

    \begin{equation}m'_{\Downarrow}= m_{\Downarrow} \label{premierePreuvelemInt19} \end{equation}

    Then:

    \begin{equation}S(\alpha,m'_{\Downarrow})=S(\alpha,m_{\Downarrow}) \label{premierePreuvelemInt20} \end{equation}

    By construction of $S$ we have for all $m$:
  \begin{equation}S(\alpha,m)=S(\alpha,m_{\Downarrow}) \label{premierePreuvelemInt2013} \end{equation}

    From \ref{premierePreuvelemInt20} and \ref{premierePreuvelemInt2013} we have:

    \begin{equation}S(\alpha,m')=S(\alpha,m) \label{premierePreuvelemInt21} \end{equation}

    Since: $|M\models_{\mathcal{C}} m'|\leq n$, we have from \ref{premierePreuvelemInt21} and the assumption of the induction in \ref{premierePreuvelemInt3}:
    \begin{equation}\forall \alpha \in {\mathcal{A}}(m).(S(\alpha,m) \subseteq S(\alpha,M))\vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{premierePreuvelemInt22} \end{equation}

    \end{itemize}

\end{itemize}

%%\end{itemize}

From \ref{premierePreuvelemInt17} and \ref{premierePreuvelemInt22}, we have for all $m$ such that $|M\models_{\mathcal{C}} m|=n+1$:
\begin{equation} M\models_{\mathcal{C}} m\Rightarrow \forall \alpha \in {\mathcal{A}}(m).(S(\alpha,m) \subseteq S(\alpha,M))\vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{premierePreuvelemInt23} \end{equation}
From \ref{premierePreuvelemInt3} and \ref{premierePreuvelemInt23} we have, for all $M \subseteq {\mathcal{M}}$ such that $M$ is well-protected:
\begin{equation}
M\models_{\mathcal{C}} m\Rightarrow \forall \alpha \in {\mathcal{A}}(m).(S(\alpha,m) \subseteq S(\alpha,M))\vee (\ulcorner K(I) \urcorner \sqsupseteq \ulcorner \alpha \urcorner) \label{premierePreuvelemInt24}
\end{equation}
Or else: \center{$S$ is full-invariant-by-intruder in ${\mathcal{C}}$.}

\end{preuve}

\begin{pre}\label{PremierelemBFSGENProofs}
$ $\\
Let  ${\mathcal{C}}=\langle{\mathcal{M}},\xi,\models,{\mathcal{K}},{\mathcal{L}}^\sqsupseteq,\ulcorner .\urcorner\rangle$ be a context  of verification.\\
\\
Let $S$ be an instance of $S_{Gen}^{EK}$.\\
\\
We have:
\center{$S$ is well-formed in ${\mathcal{C}}$.}\\

\end{pre}
$ $\\
See the proof \ref{PR25}.

\begin {preuve}\label{PR25}
$ $\\
By construction of $S$, we have:
\begin{equation}
\left\{
    \begin{array}{lll}
         S(\alpha,\{\alpha\})&=&{\mathcal{A}},\\
         &\mbox{and }& \\
         S(\alpha, {M}_1 \cup {M}_2)&=&S(\alpha, {M}_1)\cup S(\alpha,{M}_2),\\
         &\mbox{and }& \\
         S(\alpha,{M})&=&\emptyset \hspace{1mm} \mbox{, if} \hspace{1mm} \alpha \notin {\mathcal{A}}({M})\\
    \end{array}
\right.
\label{PremierepreuvelemBFSGEN1}
\end{equation}
Then: $S$ is well-formed in ${\mathcal{C}}$.
\end{preuve}


\begin{pre}\label{PremierelemBFSGENRProofs}
$ $\\
Let $S\in$ $S_{Gen}^{EK}$ and ${\mathcal{C}}$ be a context of verification.\\
Let's have a rewriting system $\rightarrow_{\xi}$ such that $\forall m \in {\mathcal{M}},\forall \alpha \in {\mathcal{A}}(m) \wedge \alpha \not \in Clear(m),$ we have: \begin{equation} \forall l \rightarrow r \in \rightarrow_{\xi},S(\alpha,r) \subseteq S(\alpha,l)\label{eqRewSystSFIBIMouchArt2} \end{equation}
We have:
%% $S$ définie en \ref{PremierelemInt1} is full-invariant-by-intruder in ${\mathcal{C}}$.\\
\center{$S$   is ${\mathcal{C}}$-reliable.}\\
\end{pre}
$ $\\
%% See the proof \ref{PR26}.
See the proof \ref{PR26}


\begin {preuve}\label{PR26}
$ $\\
Comes directly from the proposition \ref{PremierelemInt1Proofs} and the proposition \ref{PremierelemBFSGENProofs}.
\end{preuve}


\begin{defini}{$S_{MAX}^{EK}$: Selection maximum protected by an external key}\label{PremiereDefinitionSmaxProofs}
$ $\\
We define the  selection maximum protected by an external key $S_{MAX}^{EK}$ as follows:\\
\\
$
S_{MAX}^{EK}(\alpha,\alpha)={\mathcal{A}};$\begin{equation}\label{PremiereDefSmax1}\end{equation}
$S_{MAX}^{EK}(\alpha,m)=\emptyset \mbox{   if   } \alpha \not \in {\mathcal{A}}(m); $\begin{equation}\label{PremiereDefSmax2}\end{equation}
$\forall \alpha \in {\mathcal{A}}(m=f(m_1, ..., m_n)).\\
$
\begin{equation}
%\left\{
 S_{MAX}^{EK}(\alpha,m)=
    \begin{cases}
        ((\underset{1\leq i \leq n}{\cup} {\mathcal{A}}(m_i)\backslash\{\alpha\})\cap {\mathcal{I}}) {\cup} \{k^{-1}\}& \mbox{if }  f_k \in {\mathcal{E}}_{\mathcal{C}}\mbox{ and }\ulcorner {k^{-1}}\urcorner \sqsupseteq \ulcorner \alpha \urcorner \mbox{ and }\\
        & m=m_\Downarrow \mbox{ }  (a)\\
        \\
        \underset{1\leq i \leq n}{\cup} S_{MAX}^{EK}(\alpha,m_i)& \mbox{if }  f_k \in {\mathcal{E}}_{\mathcal{C}} \mbox{ and } \ulcorner {k^{-1}}\urcorner \not \sqsupseteq \ulcorner \alpha \urcorner \mbox{ and }\\
        & m=m_\Downarrow\mbox{ } (b)\\
        \\
        \underset{1\leq i \leq n}{\cup} S_{MAX}^{EK}(\alpha,m_i) & \mbox{if } f\in \overline{{\mathcal{E}}}_{\mathcal{C}} \mbox{ and } m=m_\Downarrow \mbox{ } (c) \\
        \\
        S_{MAX}^{EK}(\alpha,m_\Downarrow) &  \mbox{if } m\not=m_\Downarrow    (d)
    \end{cases}
%\right.
\label{PremiereDefSmax3}
\end{equation}
\\
and extended to sets as follows:\\
\\
$S_{MAX}^{EK}(\alpha,\{m\}\cup M)=S_{MAX}^{EK}(\alpha,\{m\}) \cup S_{MAX}^{EK}(\alpha,M)$
\begin{equation}
\label{PremiereDefSmax4}
\end {equation}
\end{defini}

$S_{MAX}^{EK}$ is the instance of the class $S_{Gen}^{EK}$ that returns for an atom in a message $m$ all its neighbors, that are principal identities, inside the protection of the external protective key $k$ in addition to its reverse form $k^{-1}$. (MAX means: the MAXimum of candidates)

\begin{defini}{$S_{EK}^{EK}$: Selection of the reverse of the protective external key only}\label{PremiereDefSExKeysProofs}
$ $\\
$ $\\
We define the selection of the reverse of the protective external key only $S_{EK}^{EK}$  as follows:\\
\\
\\
$
S_{EK}^{EK}(\alpha,\alpha)={\mathcal{A}};$\begin{equation}\label{PremiereDefSExKeys1}\end{equation}
$S_{EK}^{EK}(\alpha,m)=\emptyset \mbox{   if   } \alpha \not \in {\mathcal{A}}(m);$ \begin{equation}\label{PremiereDefSExKeys2}\end{equation}
$\forall \alpha \in {\mathcal{A}}(m=f(m_1, ..., m_n)).\\
$
\begin{equation}
%\left\{
 S_{EK}^{EK}(\alpha,m)=
    \begin{cases}
        \{k^{-1}\}& \mbox{if }  f_k \in {\mathcal{E}}_{\mathcal{C}}\mbox{ and }\ulcorner {k^{-1}}\urcorner \sqsupseteq \ulcorner \alpha \urcorner \mbox{ and }\\
        & m=m_\Downarrow \mbox{ }  (a)\\
        \\
        \underset{1\leq i \leq n}{\cup} S_{EK}^{EK}(\alpha,m_i)& \mbox{if }  f_k \in {\mathcal{E}}_{\mathcal{C}} \mbox{ and } \ulcorner {k^{-1}}\urcorner \not \sqsupseteq \ulcorner \alpha \urcorner \mbox{ and }\\
        & m=m_\Downarrow\mbox{ } (b)\\
        \\
        \underset{1\leq i \leq n}{\cup} S_{EK}^{EK}(\alpha,m_i) & \mbox{if } f\in \overline{{\mathcal{E}}}_{\mathcal{C}} \mbox{ and } m=m_\Downarrow \mbox{ } (c) \\
        \\
        S_{EK}^{EK}(\alpha,m_\Downarrow) &  \mbox{if } m\not=m_\Downarrow   (d)
    \end{cases}
%\right.
\label{PremiereDefSExKeys3}
\end{equation}
\\
and extented to sets as follows:\\
\\
$S_{EK}^{EK}(\alpha,\{m\}\cup M)=S_{EK}^{EK}(\alpha,\{m\}) \cup S_{EK}^{EK}(\alpha,M)$
\begin{equation}
\label{PremiereDefSExKeys4}
\end {equation}
\end{defini}

$S_{EK}^{EK}$ is the instance of the class $S_{Gen}^{EK}$ that returns for an atom in a message $m$ only the reverse key of the external protective key. (EK means: External Key)


\begin{defini}{$S_{N}^{EK}$: Selection of neighbors only inside the protection of an external key}\label{PremiereDefSNeighborsProofs}
$ $\\
$ $\\
We define the selection of neighbors only inside the protection of an external key $S_{N}^{EK}$  as follows:\\
\\
\\
$
S_{N}^{EK}(\alpha,\alpha)={\mathcal{A}};$\begin{equation}\label{PremiereDefSNeighbors1}\end{equation}
$S_{N}^{EK}(\alpha,m)=\emptyset \mbox{   if   } \alpha \not \in {\mathcal{A}}(m);$ \begin{equation}\label{PremiereDefSNeighbors2}\end{equation}
$\forall \alpha \in {\mathcal{A}}(m=f(m_1, ..., m_n)).\\
$
\begin{equation}
%\left\{
 S_{N}^{EK}(\alpha,m)=
    \begin{cases}
        (\underset{1\leq i \leq n}{\cup} {\mathcal{A}}(m_i)\backslash\{\alpha\}) \cap {\mathcal{I}}& \mbox{if }  f_k \in {\mathcal{E}}_{\mathcal{C}}\mbox{ and }\ulcorner {k^{-1}}\urcorner \sqsupseteq \ulcorner \alpha \urcorner \mbox{ and }\\
        & m=m_\Downarrow \mbox{ }  (a)\\
        \\
        \underset{1\leq i \leq n}{\cup} S_{N}^{EK}(\alpha,m_i)& \mbox{if }  f_k \in {\mathcal{E}}_{\mathcal{C}} \mbox{ and } \ulcorner {k^{-1}}\urcorner \not \sqsupseteq \ulcorner \alpha \urcorner \mbox{ and }\\
        & m=m_\Downarrow\mbox{ } (b)\\
        \\
        \underset{1\leq i \leq n}{\cup} S_{N}^{EK}(\alpha,m_i) & \mbox{if } f\in \overline{{\mathcal{E}}}_{\mathcal{C}} \mbox{ and } m=m_\Downarrow \mbox{ } (c) \\
        \\
        S_{N}^{EK}(\alpha,m_\Downarrow) &  \mbox{if } m\not=m_\Downarrow   (d)

    \end{cases}
%\right.
\label{PremiereDefSNeighbors3}
\end{equation}
\\
and extended to sets as follows:\\
\\
$S_{N}^{EK}(\alpha,\{m\}\cup M)=S_{N}^{EK}(\alpha,\{m\}) \cup S_{N}^{EK}(\alpha,M)$
\begin{equation}
\label{PremiereDefSNeighbors3}
\end {equation}
\end{defini}

$S_{N}^{EK}$ is the instance of the class $S_{Gen}^{EK}$ that returns only its neighbors, that are principal identities, inside the protection of the external protective key. (N means: Neighbors)\\

\begin{pre}\label{RelaibleSelectionProofs}
$ $\\
\\
$S_{MAX}^{EK}, S_{EK}^{EK}$ and $S_{N}^{EK}$ are ${\mathcal{C}}$-reliable.
\end{pre}
$ $\\
See the proof \ref{PR27}


\begin{preuve}\label{PR27}
$ $\\
\\
The selections $S_{MAX}^{EK}, S_{EK}^{EK}$ and $S_{N}^{EK}$ are instances of $S_{Gen}^{EK}$ then from the proposition \ref{PremierelemBFSGENRProofs} are ${\mathcal{C}}$-reliable.

\end{preuve}

\section{Intermediate results and proofs for Building ${\mathcal{C}}$-reliable selection-based interpretation functions}

Having defined a ${\mathcal{C}}$-reliable selection $S$, our goal now is to build ${\mathcal{C}}$-reliable selection-based interpretation functions that have the following shape:
\[
F=I\circ S.
\]
For this, it is sufficient that $I$ be a homomorphism:\\
\begin{table}[h]
   \centering
\begin{tabular}{llllll}
        &$I$&:&$({2^{\mathcal{A}}})^{\subseteq}$ &$\mapsto$& ${\mathcal{L}}^\sqsupseteq$\\
\end{tabular}
\end{table}
\\
and  $I$ respects the following order:

\begin{equation}
M_1 \subseteq M_2 \Rightarrow I(M_1) \sqsupseteq I(M_2) \label{ordrehomorphisme}
\end{equation}

\begin{comment}
\begin{preuve}\label{PR28}
$ $\\
$S$  is full-invariant-by-intruder in ${\mathcal{C}}$, then:

\begin{equation}\forall m \in {\mathcal{M}}, M\models_{\mathcal{C}} m\Rightarrow \\
\forall \alpha \in {\mathcal{A}}(m). (S(\alpha,m) \subseteq S(\alpha,M) ) \vee (\ulcorner K \urcorner \sqsupseteq \ulcorner \alpha \urcorner)
\label{preuvelemMorphisme1}
\end{equation}

Since $I$ is  a homomorphism from $({2^{\mathcal{A}}})^{\subseteq}$ to ${\mathcal{L}}^\sqsupseteq$ that respects the order \ref{ordrehomorphisme} and since ${\mathcal{L}}^\sqsupseteq$ is a lattice, we have:

\begin{equation}
\forall m \in {\mathcal{M}}, M\models_{\mathcal{C}} m\Rightarrow \forall \alpha \in {\mathcal{A}}(m). (I\circ S(\alpha,m) \sqsupseteq I\circ S(\alpha,M) ) \vee (\ulcorner K \urcorner \sqsupseteq \ulcorner \alpha \urcorner)
\label{preuvelemMorphisme2}
\end{equation}

From \ref{preuvelemMorphisme2} and the definition of $F$ we have:

\begin{equation}
\forall m \in {\mathcal{M}}. M\models_{\mathcal{C}} m\Rightarrow \forall \alpha \in {\mathcal{A}}(m). (F(\alpha,m) \sqsupseteq F(\alpha,M) ) \vee (\ulcorner K \urcorner \sqsupseteq \ulcorner \alpha \urcorner)
\label{preuvelemMorphisme3}
\end{equation}

From \ref{preuvelemMorphisme3} we have: $F$ is full-invariant-by-intruder in ${\mathcal{C}}$.\\

\end{preuve}
\end{comment}
\begin{pre}\label{preMorphismeEKRESPECTORDERProofs}
$ $\\
\\
Let $I$ be defined as follows:

%%\begin{table}[h]
%%   \centering
\begin{center}
\begin{tabular}{llllll}
        &$I$&:&$({2^{\mathcal{A}}})^{\subseteq}$ &$\mapsto$& ${\mathcal{L}}^\sqsupseteq$ \\
        &&&$M$ &$\mapsto$& $\left\{
    \begin{array}{cl}
        \top& \mbox{if } M=\emptyset \\
         \underset{\alpha \in M}{\sqcap}I(\alpha) & \mbox{if not.}
    \end{array}
\right.$ 
\end{tabular}
\end{center}
%%\end{table}
$ $\\
We have:
\center{$I$ is a homomorphism that respects the order \ref{ordrehomorphisme}.}
\end{pre}

A homomorphism $I$ as defined in \ref{preMorphismeEKRESPECTORDERProofs} ensures also the mapping from the operator "$\cup$"  to the operator "$\sqcap$" in the lattice. This mapping allows to an interpretation function to be well-formed when its associated selection is well-formed. For further details see the proof \ref{PR29}.
\normalsize

\begin{preuve}\label{PR29}
$ $\\
$\mbox{Let }M_1,M_2\mbox{ be two non-empty subsets of }({2^{\mathcal{A}}})^{\subseteq}\mbox{ such that: }$
\begin{equation}
M_1 \subseteq M_2 \label{preuvePreMorphisme1}.
\end{equation}
\\
From \ref{preuvePreMorphisme1} and since ${\mathcal{L}}^\sqsupseteq$ is a lattice, we have:
\begin{equation}
I(M_1)=\underset{\alpha \in M_1}{\sqcap}I(\alpha) \sqsupseteq \underset{\alpha \in M_2}{\sqcap}I(\alpha)=I(M_2) \label{preuvePreMorphisme2}.
\end{equation}
\\
From \ref{preuvePreMorphisme2} we have:
\begin{equation}
I(M_1) \sqsupseteq I(M_2) \label{preuvePreMorphisme3}
\end{equation}
\end{preuve}

\begin{comment}
\begin{lem}\label{lemBFFEKProofs}
$ $\\
Let $S$ be an instance of $S_{Gen}^{EK}$.\\
Let $I$ be a homomorphism as defined in \ref{preMorphismeEKRESPECTORDERProofs}.\\
\\
We have:
\[F=I\circ S \mbox{ is well-formed in } {\mathcal{C}}. \]
\end{lem}
$ $\\
See the proof \ref{PR201}.\\
\end{comment}

\begin{comment}
\begin{preuve}\label{PR201}
$ $\\
From \ref{PremiereSelectionsCreliable} and since $S$ is well-formed in $\mathcal{C}$ we have:
\begin{equation}
\left\{
    \begin{array}{lll}
         S(\alpha,\{\alpha\})&=&{\mathcal{A}},\\
         &\mbox{and }& \\
         S(\alpha, {M}_1 \cup {M}_2)&=&S(\alpha, {M}_1)\cup S(\alpha,{M}_2),\\
         &\mbox{and }& \\
         S(\alpha,{M})&=&\emptyset \hspace{1mm} \mbox{, if} \hspace{1mm} \alpha \notin {\mathcal{A}}({M})\\
    \end{array}
\right.\label{preuveFEKBFeq1}
\end{equation}
From \ref{preuveFEKBFeq1} and \ref{lemMorphismeProofs} we have:
\begin{equation} F(\alpha,\{\alpha\})=\underset{\beta \in {\mathcal{A}}({\mathcal{M}})}{\sqcap}I(\beta)=\bot\label{preuveFEKBFeq2}
\end{equation}
\\
From \ref{preuveFEKBFeq1} and \ref{lemMorphismeProofs} and since ${\mathcal{L}}^\sqsupseteq$ is a lattice we have:\\
\\
$F(\alpha, {M}_1 \cup {M}_2)=\underset{\beta \in S(\alpha,{M}_1 \cup {M}_2)}{\sqcap}I(\beta)=$
$ \underset{\beta \in S(\alpha,{M}_1)}{\sqcap}I(\beta) \sqcap \underset{\beta \in S(\alpha,{M}_2)} {\sqcap}I(\beta)=$ \begin{equation}F(\alpha, {M}_1) {\sqcap} F(\alpha, {M}_2) \label{preuveFEKBFeq3}\end{equation}
From \ref{preuveFEKBFeq1} and \ref{lemMorphismeProofs} and since ${\mathcal{L}}^\sqsupseteq$ is a lattice we have for all $\alpha \notin {\mathcal{A}}({M})$:
\begin{equation} F(\alpha,{M})=I(\emptyset)=\top \label{preuveFEKBFeq4}\end{equation}
\\
From \ref{preuveFEKBFeq2} and \ref{preuveFEKBFeq3} and \ref{preuveFEKBFeq4} we have $F$ is well-formed in $\mathcal{C}$.

\end{preuve}
\end{comment}

\begin{lem}\label{lemMorphismeProofs}
$ $\\
Let $S$ be a  full-invariant-by-intruder selection in ${\mathcal{C}}$.\\
Let $I$ be a homomorphism from $({2^{\mathcal{A}}})^{\subseteq}$ to ${\mathcal{L}}^\sqsupseteq$ that respects the order \ref{ordrehomorphisme}.\\
\\
We have:
\[F=I\circ S \mbox{ is full-invariant-by-intruder in } {\mathcal{C}}. \]
\end{lem}

A homomorphism $I$ as defined in \ref{lemMorphismeProofs} that respects  the order defined in \ref{ordrehomorphisme} ensures the mapping from the operator "$\subseteq$"  to the operator "$\sqsupseteq$" in the lattice. This mapping allows to an interpretation function to inherit the full-invariance-by-intruder from the its associated selection. For further details see the proof \ref{PR28}.

\begin{preuve}\label{PR28}
$ $\\
$S$  is full-invariant-by-intruder in ${\mathcal{C}}$, then:
\begin{equation}\forall m \in {\mathcal{M}}, M\models_{\mathcal{C}} m\Rightarrow \\
\forall \alpha \in {\mathcal{A}}(m). (S(\alpha,m) \subseteq S(\alpha,M) ) \vee (\ulcorner K \urcorner \sqsupseteq \ulcorner \alpha \urcorner)
\label{preuvelemMorphisme1}
\end{equation}
Since $I$ is  a homomorphism from $({2^{\mathcal{A}}})^{\subseteq}$ to ${\mathcal{L}}^\sqsupseteq$ that respects the order \ref{ordrehomorphisme} and since ${\mathcal{L}}^\sqsupseteq$ is a lattice, we have:
\begin{equation}
\forall m \in {\mathcal{M}}, M\models_{\mathcal{C}} m\Rightarrow \forall \alpha \in {\mathcal{A}}(m). (I\circ S(\alpha,m) \sqsupseteq I\circ S(\alpha,M) ) \vee (\ulcorner K \urcorner \sqsupseteq \ulcorner \alpha \urcorner)
\label{preuvelemMorphisme2}
\end{equation}
From \ref{preuvelemMorphisme2} and the definition of $F$ we have:
\begin{equation}
\forall m \in {\mathcal{M}}. M\models_{\mathcal{C}} m\Rightarrow \forall \alpha \in {\mathcal{A}}(m). (F(\alpha,m) \sqsupseteq F(\alpha,M) ) \vee (\ulcorner K \urcorner \sqsupseteq \ulcorner \alpha \urcorner)
\label{preuvelemMorphisme3}
\end{equation}
From \ref{preuvelemMorphisme3} we have: $F$ is full-invariant-by-intruder in ${\mathcal{C}}$.\\

\end{preuve}






\begin{lem} \label{lemBFFEKProofs}
$$$$
Let  ${\mathcal{C}}=\langle{\mathcal{M}},\xi,\models,{\mathcal{K}},{\mathcal{L}}^\sqsupseteq,\ulcorner .\urcorner\rangle$ be a context  of verification.\\
Let $S$ be an instance of $S_{Gen}^{EK}$.\\
Let $I$ be a homomorphism as defined in \ref{preMorphismeEKRESPECTORDERProofs}.\\
\\
We have:
\[F=I\circ S \mbox{ is well-formed in } {\mathcal{C}}. \]
\end{lem}
$ $\\
See the proof \ref{PR201}.\\

\begin{preuve}\label{PR201}
$$$$
Since $S$ is well-formed in $\mathcal{C}$ we have:
\begin{equation}
\left\{
    \begin{array}{lll}
         S(\alpha,\{\alpha\})&=&{\mathcal{A}},\\
         &\mbox{and }& \\
         S(\alpha, {M}_1 \cup {M}_2)&=&S(\alpha, {M}_1)\cup S(\alpha,{M}_2),\\
         &\mbox{and }& \\
         S(\alpha,{M})&=&\emptyset \hspace{1mm} \mbox{, if} \hspace{1mm} \alpha \notin {\mathcal{A}}({M})\\
    \end{array}
\right.\label{preuveFEKBFeq1}
\end{equation}
From \ref{preuveFEKBFeq1} and \ref{lemMorphismeProofs} we have:
\begin{equation} F(\alpha,\{\alpha\})=\underset{\beta \in {\mathcal{A}}({\mathcal{M}})}{\sqcap}I(\beta)=\bot\label{preuveFEKBFeq2}
\end{equation}
\\
From \ref{preuveFEKBFeq1} and \ref{lemMorphismeProofs} and since ${\mathcal{L}}^\sqsupseteq$ is a lattice we have:\\
\\
$F(\alpha, {M}_1 \cup {M}_2)=\underset{\beta \in S(\alpha,{M}_1 \cup {M}_2)}{\sqcap}I(\beta)=$
$ \underset{\beta \in S(\alpha,{M}_1)}{\sqcap}I(\beta) \sqcap \underset{\beta \in S(\alpha,{M}_2)} {\sqcap}I(\beta)=$ \begin{equation}F(\alpha, {M}_1) {\sqcap} F(\alpha, {M}_2) \label{preuveFEKBFeq3}\end{equation}
From \ref{preuveFEKBFeq1} and \ref{lemMorphismeProofs} and since ${\mathcal{L}}^\sqsupseteq$ is a lattice we have for all $\alpha \notin {\mathcal{A}}({M})$:
\begin{equation} F(\alpha,{M})=I(\emptyset)=\top \label{preuveFEKBFeq4}\end{equation}
\\
From \ref{preuveFEKBFeq2} and \ref{preuveFEKBFeq3} and \ref{preuveFEKBFeq4} we have $F$ is well-formed in $\mathcal{C}$.

\end{preuve}

\begin{lem}\label{lemCRFEKProofs}
$ $\\
Let $S$ be an instance of $S_{Gen}^{EK}$.\\
Let $I$ be a homomorphism as defined in \ref{preMorphismeEKRESPECTORDERProofs}.\\
We have:
\[F=I\circ S \mbox{ is } {\mathcal{C}}\mbox{-reliable}. \]
\end{lem}

The lemmas \ref{lemMorphismeProofs} and \ref{preMorphismeEKRESPECTORDERProofs} ensure to an interpretation function to inherit the  ${\mathcal{C}}$-reliability property from its associated selection thanks to the operators mapping of the homomorphism $I$. For further details see the proof \ref{PR202}.

\begin{preuve}\label{PR202}
$ $\\
Comes directly from \ref{lemMorphismeProofs}, \ref{preMorphismeEKRESPECTORDERProofs} and \ref{lemBFFEKProofs}.
\end{preuve}


\begin{pre}\label{preFCREKProofs}
$ $\\
Let $\psi$ be a homomorphism defined as follows:
%%\begin{table}[h]
%%  \centering
%%Let $\psi$ be a homomorphism defined as follows:
\begin{center}
\begin{tabular}{lrllll}
        &$\psi$&:&$({2^{\mathcal{A}}})^{\subseteq}$ &$\mapsto$& ${\mathcal{L}}^\sqsupseteq$ \\
        &&&$M$ &$\mapsto$&$\left\{
    \begin{array}{cl}   
        \top& \mbox{if } M=\emptyset  \\
         \underset{\alpha \in M}{\sqcap}\psi(\alpha) & \mbox{if not.}    
    \end{array}
\right.$\\
\\
&such that:&\multicolumn{4}{c}{$\psi(\alpha)=\left\{
    \begin{array}{ll}
        \{\alpha\} & \mbox{if } \alpha \in {\mathcal{I}} \mbox{ (Principal Identities) }  \\
        \ulcorner\alpha\urcorner & \mbox{if not.}
    \end{array}
\right.$}
\end{tabular}
\end{center}
%%\end{table}
\mbox{ We have: }$F_{MAX}^{EK}= \psi\circ S_{MAX}^{EK}$, $F_{EK}^{EK}=\psi\circ S_{EK}^{EK}$ and $F_{N}^{EK}=\psi\circ S_{N}^{EK}$ are  ${\mathcal{C}}$-reliable.
\end{pre}

The proposition \ref{preFCREKProofs} gives the way to transform the elements returned by a selection to security levels.
$ $\\
\\
See the proof \ref{PR203}

\begin{preuve}\label{PR203}
$ $\\
According to the proposition \ref{preFCREKProofs} we have: \begin{equation}\psi \mbox{ is a homomorphism as defined in the proposition } \ref{preMorphismeEKRESPECTORDERProofs} \label{eq1preuvepreFCREK}\end{equation}
From \ref{eq1preuvepreFCREK} and  the lemmas \ref{lemMorphismeProofs} and \ref{lemBFFEKProofs} and the proposition  \ref{PremierelemInt1Proofs}  we have directly:
$F_{MAX}^{EK}$, $F_{EK}^{EK}$ and $F_{N}^{EK}$ are  ${\mathcal{C}}$-reliable.
\end{preuve}
%%\pagebreak

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Intermediate results and proofs for Witness-Functions}
%%% preuves du chapitre de construction des selection et fonctions fiables.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{pre}{}\label{WCReliableArtNouchArticleProofs}
$ $\\
Let ${\mathcal{W}}_{p,F}$ be a witness-function inside the protection of an external key.\\
We have:
\center{${\mathcal{W}}_{p,F}$ inherits reliability from $F$}
\end{pre}
$ $\\

The selection associated with a witness-function inside the protection of an external key is the union of selections  associated with the interpretation function $F$ restricted to derivative messages. It is easy to verify that a witness-function is  by construction well-formed. For the full-invariance-by-intruder property, since the derivation just removes variables and since each selection in the union returns a subset among acceptable candidates, then the union itself returns a subset among acceptable candidates (the union of subsets is a subset). Therefore, the selection associated with a witness-function remains an instance of the class $S_{Gen}^{EK}$ and so full-invariant-by-intruder. Since the witness-function is the composition of the homomorphism associated with $F$ and an instance of the class $S_{Gen}^{EK}$, then it is reliable. \\
\\
See the proof \ref{PR31}

\begin{preuve}{}{\label{PR31}}
$ $\\
Let $F$ be a ${\mathcal{C}}$-reliable interpretation function associated with a selection $S$ of the class $S_{Gen}^{EK}$ and $\psi$ the homomorphism such that $F=\psi \circ S$.\\
\\
Let $m\in$ ${\mathcal{M}}_p^{\mathcal{G}}$.\\
\\
Let $S_{\mathcal{W}}$ the selection associated with ${\mathcal{W}}_{p,F}$ in $p$.\\
\\
Since $\psi$ is a homomorphism then: \begin{equation}{\mathcal{W}}_{p,F}=\psi \circ S_{\mathcal{W}}\label{eq1preuveWisCReliable}.\end{equation}
where $S_{\mathcal{W}}$ is defined on all closed message $m\sigma$ as follows:\\
\\
$S_{\mathcal{W}}(\alpha,\alpha)={\mathcal{A}};$\begin{equation}\label{eq2preuveWisCReliable}\end{equation}
$S_{\mathcal{W}}(\alpha,m\sigma)=\emptyset \mbox{   if   } \alpha \not \in {\mathcal{A}}(m\sigma);$ \begin{equation}\label{eq3preuveWisCReliable}\end{equation}
$\forall \alpha \in {\mathcal{A}}(m\sigma=f(m_1, ..., m_n)).$\\
%%$\\
%%\begin{tabular}{ll}
 %%  $S_{\mathcal{W}}(\alpha,m\sigma)=\underset{\overset {m' \in {\mathcal{M}}_p^{\mathcal{G}}}{\exists \sigma' \in \Gamma.m'\sigma' = m \sigma }}{\cup} S(\alpha, \partial [\underline{\alpha}] m'\sigma') $ & $\mbox{if }  f_k \in {\mathcal{E}}_{\mathcal{C}}$\\
%%   &$\mbox{and }\ulcorner {k^{-1}}\urcorner \sqsupseteq \ulcorner \alpha \urcorner$ \\
 %%  & $\mbox{and }m\sigma={m\sigma}_\Downarrow$
%% \end{tabular}
%%\begin{equation}\label{eq4preuveWisCReliable}\end{equation}
\begin{equation}
%\left\{
S_{\mathcal{W}}(\alpha,m\sigma)=
    \begin{cases}
\underset{\overset {m' \in {\mathcal{M}}_p^{\mathcal{G}}}{\exists \sigma' \in \Gamma.m'\sigma' = m \sigma }}{\cup} S(\alpha, \partial [\underline{\alpha}] m'\sigma') & \mbox{if }  f_k \in {\mathcal{E}}_{\mathcal{C}} \mbox{ and }\ulcorner {k^{-1}}\urcorner \sqsupseteq \ulcorner \alpha \urcorner \mbox{ and }\\ &\ulcorner {k^{-1}}\urcorner \sqsupseteq \ulcorner \alpha \urcorner   (a)\\
\\
 \underset{1\leq i \leq n}{\cup} S_{\mathcal{W}}(\alpha,m_i)& \mbox{if }  f_k \in {\mathcal{E}}_{\mathcal{C}} \mbox{ and } \ulcorner {k^{-1}}\urcorner \not \sqsupseteq \ulcorner \alpha \urcorner \mbox{ and }\\
        & m\sigma={m\sigma}_\Downarrow\mbox{ } (b)\\
        \\
        \underset{1\leq i \leq n}{\cup} S_{\mathcal{W}}(\alpha,m_i) & \mbox{if } f\in \overline{{\mathcal{E}}}_{\mathcal{C}} \mbox{ and } m\sigma={m\sigma}_\Downarrow \mbox{ } (c) \\
        \\
        S_{\mathcal{W}}(\alpha,{m\sigma}_\Downarrow) &  \mbox{if } m\sigma\not={m\sigma}_\Downarrow   (d)

    \end{cases}
%\right.
\label{eq5preuveWisCReliable}
\end{equation}
\\
and extended to sets as follows:\\
\\
$S_{\mathcal{W}}(\alpha,\{m\sigma\}\cup M)=S_{\mathcal{W}}(\alpha,\{m\sigma\}) \cup S(\alpha,M).$
\begin{equation}
\label{eq6preuveWisCReliable}
\end {equation}

\begin{itemize}
  \item[$\bullet$] Under the conditions \ref{eq2preuveWisCReliable}, \ref{eq3preuveWisCReliable}, \ref{eq5preuveWisCReliable}(b), \ref{eq5preuveWisCReliable}(c)and \ref{eq5preuveWisCReliable} (d) we have:\\
	\begin{equation}S_{\mathcal{W}}\mbox{ respects the  definition of an instance of the class 		}S_{Gen}^{EK} \label{eq7preuveWisCReliable} \end{equation} 
  \item [$\bullet$] Under the condition \ref{eq5preuveWisCReliable} (a), we have for all $\alpha \in {\mathcal{A}}(m\sigma=f(m_1, ..., m_n))$:\\
\begin{equation}S_{\mathcal{W}}(\alpha,m\sigma)=\underset{\overset {m' \in {\mathcal{M}}_p^{\mathcal{G}}}{\exists \sigma' \in \Gamma.m'\sigma' = m \sigma }}{\cup} S(\alpha, \partial [\underline{\alpha}] m'\sigma') \label{eq8preuveWisCReliable} \end{equation} 
Since derivation removes atoms, we have:
\begin{equation} S(\alpha, \partial [\underline{\alpha}] m'\sigma') \subseteq S(\alpha,m'\sigma')\label{eq9preuveWisCReliable} \end{equation} 
From  \ref{eq8preuveWisCReliable} and  \ref{eq9preuveWisCReliable} we have:
\begin{equation}S_{\mathcal{W}}(\alpha,m\sigma) \subseteq \underset{\overset {m' \in {\mathcal{M}}_p^{\mathcal{G}}}{\exists \sigma' \in \Gamma.m'\sigma' = m \sigma }}{\cup} S(\alpha, m'\sigma')\label{eq10preuveWisCReliable} \end{equation} 
But we have: 
\begin{equation} \underset{\overset {m' \in {\mathcal{M}}_p^{\mathcal{G}}}{\exists \sigma' \in \Gamma.m'\sigma' = m \sigma }}{\cup} S(\alpha, m'\sigma')=\underset{\overset {m' \in {\mathcal{M}}_p^{\mathcal{G}}}{\exists \sigma' \in \Gamma.m'\sigma' = m \sigma }}{\cup} S(\alpha, m\sigma)=S(\alpha, m\sigma)\label{eq11preuveWisCReliable} \end{equation} 
Since $S$ is an instance of the class $S_{Gen}^{EK}$, we have:
\begin{equation} S(\alpha, m\sigma)\subseteq (\underset{1\leq i \leq n}{\cup} {\mathcal{A}}(m_i){\cup} \{k^{-1}\})\backslash\{\alpha\}\label{eq12preuveWisCReliable} \end{equation} 
From $\ref{eq10preuveWisCReliable}, \ref{eq11preuveWisCReliable}$ and $\ref{eq12preuveWisCReliable}$, we have:
\begin{equation} S_{\mathcal{W}}(\alpha, m\sigma)\subseteq (\underset{1\leq i \leq n}{\cup} {\mathcal{A}}(m_i){\cup} \{k^{-1}\})\backslash\{\alpha\}\label{eq13preuveWisCReliable} \end{equation} 
Or else, under the condition \ref{eq5preuveWisCReliable} (a):
\begin{equation} S_{\mathcal{W}} \mbox{ respects the definition of an instance of the class 		}S_{Gen}^{EK}\label{eq14preuveWisCReliable} \end{equation} 
\end{itemize}
From \ref{eq7preuveWisCReliable} and \ref{eq14preuveWisCReliable} we have:
\begin{equation} S_{\mathcal{W}} \mbox{ is an instance of the class 		}S_{Gen}^{EK}\label{eq15preuveWisCReliable} \end{equation} 
Since $\psi$, the homomorphism associated with $F$, is as defined in \ref{preMorphismeEKRESPECTORDERProofs} and from \ref{eq1preuveWisCReliable}, \ref{eq15preuveWisCReliable} and the lemma \ref{lemCRFEKProofs} we have:
\center{ ${\mathcal{W}}_{p,F}$ is ${\mathcal{C}}$-reliable.}
\end{preuve}
\begin{comment}
\begin{preuve}{}\label{preuvePAT}

$ $\\
\\
Suppose we have:\\
\\
$\forall R.r \in R_G(p), \forall \alpha \in {\mathcal{A}}{(r^+ )}$ we have:\\
\begin{equation}
\underset{\overset {m' \in {\mathcal{M}}_p^{\mathcal{G}}}{\exists \sigma' \in \Gamma.m'\sigma' = r^+ \sigma' }}{\sqcap} F(\alpha, \partial[\underline{\alpha}] m'\sigma') \sqsupseteq \ulcorner \alpha \urcorner \sqcap F(\alpha,\partial [\underline{\alpha}]R^-) \label{preuvtheDernier4}
\end{equation}
From \ref{corBounds} and since  ${\mathcal{L}}^\sqsupseteq$ is a lattice we have for all $\sigma \in \Gamma$:
\begin{equation}
{\mathcal{W}}_{p,F}(\alpha, r^+\sigma )\sqsupseteq\underset{\overset {m' \in {\mathcal{M}}_p^{\mathcal{G}}}{\exists \sigma' \in \Gamma.m'\sigma' = r^+ \sigma' }}{\sqcap} F(\alpha, \partial [\underline{\alpha}]m'\sigma') \label{preuvtheDernier2}\end{equation}
$$\mbox{and}$$ 
\begin{equation}
 \ulcorner \alpha \urcorner \sqcap F(\alpha,\partial[\underline{\alpha}] R^-) \sqsupseteq  \ulcorner \alpha \urcorner \sqcap {\mathcal{W}}_{p,F}(\alpha,R^-\sigma )   \label{preuvtheDernier3}\end{equation}
From \ref{preuvtheDernier4}, \ref{preuvtheDernier2} and \ref{preuvtheDernier3} we have:
\begin{equation}
{\mathcal{W}}_{p,F}(\alpha, r^+\sigma )\sqsupseteq \ulcorner \alpha \urcorner \sqcap {\mathcal{W}}_{p,F}(\alpha,R^-\sigma )\label{preuvtheDernier1}\end{equation}
From \ref{WCReliable} ${\mathcal{W}}_{p,F}$ is  ${\mathcal{C}}$-reliable we have from the theorem \ref{mainTh} and \ref{preuvtheDernier1}: 
\[p \mbox{ is correct with respect to the secrecy property.}\]

\end{preuve}
\end{comment}

\begin{lem}{}\label{corBoundsArtmouchArticleProofs}
$ $\\
Let $m\in{\mathcal{M}}_p^{\mathcal{G}}$ and ${\mathcal{W}}_{p,F}$ be a witness-function inside the protection of an external key.\\
$\forall \sigma \in \Gamma, \forall \alpha \in {\mathcal{A}}({\mathcal{M}}_p)$ we have:
\[F(\alpha,\partial [\overline{\alpha}] m) \sqsupseteq {\mathcal{W}}_{p,F}(\alpha,m\sigma) \sqsupseteq \underset{\overset {m' \in {\mathcal{M}}_p^{\mathcal{G}}}{\exists \sigma' \in \Gamma.m'\sigma' = m \sigma' }}{\sqcap} F(\alpha, \partial [\overline{\alpha}]m'\sigma')\]
\end{lem}

The upper bound of a witness-function estimates the security level of a given atom $\alpha$ in a given closed message $m\sigma$ from one \textit{confirmed} source $m$, the witness-function itself estimates it from the \textit{exact} sources of $m\sigma$  (i.e. when the protocol is executed), and the lower bound estimates it from all \textit{likely} sources of $m\sigma$ (i.e. the messages that can be unified with $m$ in ${\mathcal{M}}_p^{\mathcal{G}}$). The unification in the lower bound "hunts" all the candidates from all the \textit{likely} sources of the closed message in the protocol. Please notice that the upper bound and the lower bound of the Witness-Function ${\mathcal{W}}_{p,F}$ do not depend on $\sigma$.
$ $\\
\\
See the proof \ref{PRcorBounds}

%%\begin{comment}
\begin{preuve}{}\label{PRcorBounds}
$ $\\
For any $\sigma \in \Gamma$ we have:
%%$ $\\
\begin{itemize}
  \item [$\bullet$] $F(\alpha,\partial[\overline{\alpha}] m)\subseteq {\mathcal{W}}_{p,F}(\alpha,m\sigma)$: 
%%puisque $m$ est naturellement dans l'ensemble de calcul de ${\mathcal{W}}_{p,F}$.\\
since $m$ is obviously one element of the set $\{m' \in {\mathcal{M}}_p^{\mathcal{G}}|\exists \sigma' \in \Gamma.m'\sigma' = m \sigma\}$ of calculation of ${\mathcal{W}}_{p,F}(\alpha,m\sigma)$  (i.e. $m$ is a trivial source of $m\sigma$) 
%% and $F(\alpha,\partial[\overline{\alpha}] m)= F(\alpha,\partial[\overline{\alpha}] m\sigma)$ 
and since $ F(\alpha,\partial[\overline{\alpha}] m\sigma)$ does not depend on $\sigma$ because, by construction, it depends only on the static part of $m$ (denoted simply by $F(\alpha,\partial[\overline{\alpha}] m)$).
  \item [$\bullet$] ${\mathcal{W}}_{p,F}(\alpha,m\sigma)\subseteq \underset{\overset {m' \in {\mathcal{M}}_p^{\mathcal{G}}}{\exists \sigma' \in \Gamma.m'\sigma' = m \sigma' }}{\cup} F(\alpha, \partial [\overline{\alpha}]m'\sigma')$: 
since for all $m \in {\mathcal{M}}_p^{\mathcal{G}}$ the set $\{m' \in {\mathcal{M}}_p^{\mathcal{G}}|\exists \sigma' \in \Gamma.m'\sigma' = m \sigma'\}$ (unifications) is obviously larger than the set $\{m' \in {\mathcal{M}}_p^{\mathcal{G}}|\exists \sigma' \in \Gamma.m'\sigma' = m \sigma\}$ of sources of $m\sigma$ in ${\mathcal{M}}_p^{\mathcal{G}}$.\\
From these two facts and since ${\mathcal{L}}^\sqsupseteq$ is a lattice, we have: \[F(\alpha,\partial [\overline{\alpha}] m) \sqsupseteq {\mathcal{W}}_{p,F}(\alpha,m\sigma) \sqsupseteq \underset{\overset {m' \in {\mathcal{M}}_p^{\mathcal{G}}}{\exists \sigma' \in \Gamma.m'\sigma' = m \sigma' }}{\sqcap} F(\alpha, \partial [\overline{\alpha}]m'\sigma')\]
%%puisque l'ensemble de messages unifiables est plus large que l'ensemble de sources.\\
\end{itemize}
%%$\blackbox$
\end{preuve}
%%\end{comment}

%%\begin{comment}
\begin{thm}(Protocol analysis with a Witness-Function)\label{PATmouchArticleProofs}
$ $\\
$ $\\
%% Let $p$ be a protocol.\\ \\
%% Let $F$ be a ${\mathcal{C}}-$reliable interpretation function.\\
%%Soit ${\mathcal{W}}_{p,F}$ une fonction témoin.\\
Let ${\mathcal{W}}_{p,F}$ be a witness-function inside the protection of an external key.\\ \\
A sufficient condition of correctness of $p$ with respect to the secrecy property is:\\
\\
$\forall R.r \in R_G(p), \forall \alpha \in {\mathcal{A}}{(r^+ )}$ we have:\\
\[
\underset{\overset {m' \in {\mathcal{M}}_p^{\mathcal{G}}}{\exists \sigma' \in \Gamma.m'\sigma' = r^+ \sigma' }}{\sqcap} F(\alpha, \partial[\overline{\alpha}] m'\sigma') \sqsupseteq \ulcorner \alpha \urcorner \sqcap F(\alpha,\partial[\overline{\alpha}] R^-)
\]\end{thm}
%%\end{comment}
$ $\\
\\

The result in the theorem \ref{PATmouchArticleProofs} comes directly from the proposition \ref{WCReliableArtNouchArticleProofs}, the lemma \ref{corBoundsArtmouchArticleProofs} and the theorem \ref{mainThmouchArticleProofs}. Thanks to the independence of the criterion stated by the theorem \ref{PATmouchArticleProofs} of all substitutions, any decision made on the generalized roles can be exported to valid traces. %%Thanks to the independence 
$ $\\
\\
See the proof \ref{PATmouchArticle}

\begin{preuve}{}\label{PATmouchArticle}
$ $\\
$\mbox{ Suppose we have:                         }\forall R.r \in R_G(p), \forall \alpha \in {\mathcal{A}}{(r^+ )}$
\begin{equation}
\underset{\overset {m' \in {\mathcal{M}}_p^{\mathcal{G}}}{\exists \sigma' \in \Gamma.m'\sigma' = r^+ \sigma' }}{\sqcap} F(\alpha, \partial[\overline{\alpha}] m'\sigma') \sqsupseteq \ulcorner \alpha \urcorner \sqcap F(\alpha,\partial [\overline{\alpha}]R^-) \label{LapreuvDuDernier4}
\end{equation}
From the lemma \ref{corBoundsArtmouchArticleProofs} and since  ${\mathcal{L}}^\sqsupseteq$ is a lattice we have for all $\sigma \in \Gamma$:
\begin{equation}
\forall \alpha \in {\mathcal{A}}({\mathcal{M}}_p).{\mathcal{W}}_{p,F}(\alpha, r^+\sigma )\sqsupseteq\underset{\overset {m' \in {\mathcal{M}}_p^{\mathcal{G}}}{\exists \sigma' \in \Gamma.m'\sigma' = r^+ \sigma' }}{\sqcap} F(\alpha, \partial [\overline{\alpha}]m'\sigma') \label{LapreuvDuDernier2}\end{equation}
$$\mbox{and}$$ 
\begin{equation}
\forall \alpha \in {\mathcal{A}}({\mathcal{M}}_p).\ulcorner \alpha \urcorner \sqcap F(\alpha,\partial[\overline{\alpha}] R^-) \sqsupseteq  \ulcorner \alpha \urcorner \sqcap {\mathcal{W}}_{p,F}(\alpha,R^-\sigma )   \label{LapreuvDuDernier3}\end{equation}
From \ref{LapreuvDuDernier4}, \ref{LapreuvDuDernier2} and \ref{LapreuvDuDernier3} we have:
\begin{equation}
\forall \alpha \in {\mathcal{A}}(r^+\sigma).{\mathcal{W}}_{p,F}(\alpha, r^+\sigma )\sqsupseteq \ulcorner \alpha \urcorner \sqcap {\mathcal{W}}_{p,F}(\alpha,R^-\sigma )\label{LapreuvDuDernier1}\end{equation}
From the proposition \ref{WCReliableArtNouchArticleProofs}  ${\mathcal{W}}_{p,F}$ is  ${\mathcal{C}}$-reliable, then we have from the theorem \ref{mainThmouchArticleProofs} and \ref{LapreuvDuDernier1}: 
\[p \mbox{ is correct with respect to the secrecy property}\]
\end{preuve}
